Quantum State Obfuscation from Classical Oracles

A major unresolved question in quantum cryptography is whether it is possible to obfuscate arbitrary quantum computation. Indeed, there is much yet to understand about the feasibility of quantum obfuscation even in the classical oracle model, where one is given for free the ability to obfuscate any classical circuit. In this work, we develop a new array of techniques that we use to construct a quantum state obfuscator, a powerful notion formalized recently by Coladangelo and Gunn (arXiv:2311.07794) in their pursuit of better software copy-protection schemes. Quantum state obfuscation refers to the task of compiling a quantum program, consisting of a quantum circuit $C$ with a classical description and an auxiliary quantum state $\ket{\psi}$, into a functionally-equivalent obfuscated quantum program that hides as much as possible about $C$ and $\ket{\psi}$. We prove the security of our obfuscator when applied to any pseudo-deterministic quantum program, i.e. one that computes a (nearly) deterministic classical input / classical output functionality. Our security proof is with respect to an efficient classical oracle, which may be heuristically instantiated using quantum-secure indistinguishability obfuscation for classical circuits. Our result improves upon the recent work of Bartusek, Kitagawa, Nishimaki and Yamakawa (STOC 2023) who also showed how to obfuscate pseudo-deterministic quantum circuits in the classical oracle model, but only ones with a completely classical description. Furthermore, our result answers a question of Coladangelo and Gunn, who provide a construction of quantum state indistinguishability obfuscation with respect to a quantum oracle. Indeed, our quantum state obfuscator together with Coladangelo-Gunn gives the first candidate realization of a ``best-possible'' copy-protection scheme for all polynomial-time functionalities.

==> notes.tex <==
\section{Publicly-Verifiable Quantum Authentication Scheme}

References for quantum authentication: \cite{1181969,aharonov2017interactive,C:BroGutSte13,dulek2018quantum}

A quantum authentication scheme (QAS) is defined by a keyed unitary $E_k^{\regM\regA}$ that operates on a message register $\regM$ and an auxiliary register $\regA$. The encoding operation is an isometry $\Enc_k : \regM \to \regM\regA$ defined by \[\Enc_k: \rho^\regM \to E_k(\rho^\regM \otimes \ketbra{0}{0}^\regA)E_k^\dagger.\] Define the accept projector \[\Pi_{k}^{\regM\regA} \coloneqq E_k(\bbI^\regM \otimes \ketbra{0}{0}^\regA)E_k^\dagger,\] and the decoding operation $\Dec_k : \regM\regA \to \regM$  \[\Dec_k : \overline{\rho} \to \Tr_\regA(\Pi_k\overline{\rho}\Pi_k) + \Tr_{\regM\regA}((\bbI-\Pi_k)\overline{\rho}(\bbI-\Pi_k)) \otimes \ketbra{\bot}{\bot}^\regM.\] The standard authentication security stipulates that for any attack unitary $U^{\regM\regA}$, there exists $p_{\mathsf{acc}} \in [0,1]$ such that\footnote{For simplicity, we are not considering a side register that could even be entangled with the message register, but we will add this later.} \[\big\|\E_k\left[\Dec_k \circ U \circ \Enc_k \right] - (p_{\mathsf{acc}}\bbI + (1-p_{\mathsf{acc}})(\Tr_\regM \otimes \ketbra{\bot}{\bot})\big\|_\diamond = \negl.\] We will be interested in a strengthening of this property that allows the adversary to have oracle access to the accept projector of the QAS. That is, for attack unitary $U^{\regM\regA}$, there exists $p_{\mathsf{acc}} \in [0,1]$ such that \[\big\|\E_k\left[\Dec_k \circ U^{\{\Pi_k,\bbI-\Pi_k
\}} \circ \Enc_k \right] - (p_{\mathsf{acc}}\bbI + (1-p_{\mathsf{acc}})(\Tr_\regM \otimes \ketbra{\bot}{\bot})\big\|_\diamond = \negl.\] The notation $U^{\{\Pi_k,\bbI-\Pi_k\}}$ means that $U$ can repeatedly submit a state on registers $\regM\regA$ to its oracle, which applies the projective measurement $\{\Pi_k,\bbI-\Pi_k\}$ and then returns the resulting state.

\subsection{Construction}

\begin{itemize}
    \item To authenticate $m$ qubits, the key $k$ consists of $(S,\Delta,\{x_i,z_i\}_{i \in [m]})$, where $S \subset \bbF_2^{2n+1}$ is a uniformly random $n$-dimensional subspace, $\Delta \gets \bbF_2^{2n+1} \setminus S$, and each $x_i,z_i \gets \bbF_2^{2n+1}$.
    \item The unitary $E_k$ is defined as follows: 
    \[E_k \coloneqq \left(X^{x_1}Z^{z_1} \otimes \dots \otimes X^{x_m}Z^{z_m}\right) \left(C_{S,\Delta}^{\otimes m}\right),\] where  $C_{S,\Delta}$ is a unitary completion of the map \[\ket{0,0^{2n}} \to \ket{S}, \\\, \ket{1,0^{2n}} \to \ket{S+\Delta}.\]  
    \item Notation: Given $(S,\Delta)$, let $S_\Delta \coloneqq S \cup S+\Delta$, $\widehat{S} \coloneqq S_\Delta^\bot$, and $\widehat{\Delta}$ be a canonical choice of vector such that $S^\bot = \widehat{S} \cup \widehat{S} + \widehat{\Delta}$. We will also sometimes write $\widehat{S}_{\widehat{\Delta}} \coloneqq S^\bot = \widehat{S} \cup \widehat{S} + \widehat{\Delta}$.
    \item It can be shown that \[\Pi_k = \left(\Pi[\widehat{S}_{\widehat{\Delta}} + z_1] \otimes \dots \otimes \Pi[\widehat{S}_{\widehat{\Delta}} + z_m]\right) H^{\otimes m(2n+1)} \left(\Pi[S_\Delta + x_1]\otimes \dots \otimes \Pi[S_\Delta + x_m]\right),\] where for an affine subspace $A$, $\Pi[A]$ projects onto vectors in $A$.
\end{itemize}

\subsection{Security}

\begin{claim}\label{claim:QAS}
The above scheme is a publicly-verifiable QAS.
\end{claim}

\begin{proof}
    Outline: (will fill in details later)
    \begin{itemize}
        \item It suffices to show that security holds when we give the adversary (quantum-accessible) access to the classical oracles $\{\Pi[S_\Delta+x_i],\Pi[\widehat{S}_{\widehat{\Delta}} + z_i]\}_{i \in [m]}$.
        \item Sample random superspaces $T \supset S_\Delta$ and $R \supset \widehat{S}_{\widehat{\Delta}}$ of dimension $3n/2 + 1$, and give the adversary oracle access to $\{\Pi[T+x_i],\Pi[R + z_i]\}_{i \in [m]}$ instead. This will only introduce a $\negl(\secp)$ trace distance.
        \item Fix a choice of $R^\bot \subset T$, where $R$ has dimension $n/2$ and $T$ has dimension $3n/2 + 1$, and let $\co(T),\co(R)$ be sets of coset representatives of $T$ and $R$. We can then sample $S,\Delta$ uniformly at random such that $R^\bot \subset S \subset S_\Delta \subset T$, and sample each $x_i,z_i$ in two parts: $x_i = x_{i,T} + x_{i,\co(T)}$ and $z_i = z_{i,R} + z_{i,\co(R)}$, where $x_{i,T} \gets T$ and $x_{i,\co(T)} \gets \co(T)$ (and analogously for $z_i$).
        \item We give out $(T,R,x_{1,\co(T)},z_{1,\co(R)},\dots,x_{m,\co(T)},z_{m,\co(R)})$ in the clear so that the adversary can implement the oracles by itself. We apply the Pauli twirl within the space defined by $T,R$ using the randomness of $x_{i,T}$ and $z_{i,R}$ to reduce the adversary's attack to a mixture over fixed Pauli attacks $X^x Z^z$ for $x \in T,z \in R$. Then, we use the randomness of $S$ and $\Delta$ to show that any fixed Pauli attack fails to tamper with the encoded qubit except with negligible probability. 
    \end{itemize}
\end{proof}

\subsection{Random Measurement Oracle}

We will consider giving the adversary access to an additional oracle that can be used to perform a measurement on authenticated data. Crucially, the outputs of this oracle will be random labels rather than fixed bit strings. For example, a standard basis measurement on the first register can be performed with an oracle implementing the following map: $S+x_1 \to \ell_0, S+\Delta+x_1 \to \ell_1$, where $\ell_0$ and $\ell_1$ are random strings.

Given an authenticated state and a random measurement oracle, clearly the adversary can break the security of the authentication scheme by using the oracle to perform a measurement on the state. However, suppose that the oracle takes an additional input, and only responds if that input is in some set $K$. That is, we define the oracle as follows.

\[O(k,s)  \to \begin{cases}\ell_0 \text{ if $k \in K, s \in S+x_1$} \\ \ell_1 \text{ if $k \in K, s \in S+\Delta + x_1$} \\ \bot \text{ else} \end{cases}.\]

Then, we will claim that some $k \in K$ can be extracted from any adversary that breaks the authentication scheme. We discuss more about this claim in the next section.

\subsection{Toy Problem}

Given a random subspace state $\ket{A}$, an authenticated 0 state $X^xZ^z\ket{S}$, and access to the oracle

\[O(a,s) \to \begin{cases}H(a,0) \text{ if } a \in A^\bot, s \in \widehat{S} \\ H(a,1) \text{ if } a \in A^\bot, s \in \widehat{S} + \widehat{\Delta} \\ \bot \text { else}\end{cases}\] where $H$ is a random oracle, can we show that any adversary outputs $a \in A$ and (a state with noticeable overlap with) $X^xZ^z\ket{S+\Delta}$ with only negligible probability?

\begin{itemize}
    \item In general, we will want to show that the above QAS scheme remains secure in the following setting. A signature token key will be included as part of the authenticated state, and the decoding operation will only accept if given a signature of 0. But the adversary will additionally have access to an oracle that can be used to maul the state in some way (e.g. perform a measurement in the Hadamard basis as in the example above) that will only work when given a signature of 1. This setting is relevant to our obfuscation candidate (see \cref{sec:obfuscation}).
    \item The example above is a special case where we authenticate the 0 state and ask the adversary to produce an authenticated 1 state.
    \item Note that it is easy to output \emph{either} $a \in A$ \emph{or} a state close to $X^xZ^z\ket{S+\Delta}$. For the latter, first apply Hadamard to both $\ket{A}$ and $X^x Z^z \ket{S}$, measure $a \in A^\bot$, query the oracle and measure the output to collapse the state to either $X^z Z^x \ket{\widehat{S}}$ or $X^z Z^x \ket{\widehat{S} + \widehat{\Delta}}$, and then apply Hadamard to obtain either $X^x Z^z (\ket{S} + \ket{S+\Delta})$ or $X^x Z^z (\ket{S} - \ket{S+\Delta})$, both of which have 1/2 overlap with the authenticated 1 state.
    \item One idea for an attack would be to not fully collapse the state, for example only measuring the first bit of the output of $H$, and otherwise leaving $\ket{A^\bot}$ in superposition. For simplicity, assume that the first bit of $H(a,0)$ is always opposite the first bit of $H(a,1)$, and let $A^\bot_b$ be the set of $a \in A^\bot$ such that the first bit of $H(a,0)$ is $b$. Then after measuring this bit, the remaining state can be written as 
    \begin{align*}
        &\ket{A^\bot_0} \otimes X^z Z^x\ket{\widehat{S}} + \ket{A^\bot_1} \otimes X^z Z^x\ket{\widehat{S} + \widehat{\Delta}} \\ 
        &\xrightarrow{\bbI^{\otimes n} \otimes H^{\otimes n}} \ket{A^\bot_0} \otimes X^x Z^z (\ket{S} + \ket{S+\Delta}) + \ket{A^\bot_1} \otimes X^x Z^z (\ket{S} - \ket{S+\Delta}) \\
        &= \ket{A^\bot} \otimes X^x Z^z \ket{S} + \left(\ket{A^\bot_0} - \ket{A^\bot_1}\right) \otimes X^x Z^z \ket{S+\Delta},
    \end{align*}
    so the part of the adversary's state that contains $X^xZ^z\ket{S+\Delta}$ is tensored with $\ket{A^\bot_0} - \ket{A^\bot_1}$, which is $\ket{A^\bot}$ with a uniformly random $+1/-1$ phase. Measuring such a state in the Hadamard basis should fail to produce $a \in A$, since the random phase messes up the interference:
    \[H^{\otimes n}\sum_{a \in A^\bot}(-1)^{f(a)}\ket{a} = \sum_v\left(\sum_{a \in A^\bot}(-1)^{v \cdot a + f(a)}\right)\ket{v}.\]
\end{itemize}

\begin{conjecture} Take any adversary in the above game, implement the random oracle as a compressed oracle, project their second output register onto the state $X^xZ^z\ket{S+\Delta}$, and then measure the database register. Then there is only a negligible probability that the projection accepts but the measured database does not contain an $a \in A^\bot$. In other words, whenever the adversary succesfully mauls the state, the database will certainly contain a recording of some $a \in A^\bot$.
\end{conjecture}

\begin{itemize}
    \item In particular, this would imply that conditioned on the projection succeeding, the adversary's first output register can only be in the support of $A$ with negligible probability. Otherwise there exists a reduction that given $\ket{A}$ and oracle access to a membership check for $A^\bot$, outputs $(a,a') \in A \times A^\bot$ with noticeable probability, which is impossible.
    \item For now let's consider the random oracle to only have a single bit of output. We'll use a standard compressed oracle, so the empty database $\ket{\emptyset}$ corresponds to $\ket{+}\dots\ket{+}$, and a database corresponds to the set of registers that are $\ket{-}$. A query on some unitialized value $x$ with output register set to 0 evolves as \[\ket{0}\ket{+} \to \ket{00}+\ket{11} = \ket{0}(\ket{+} + \ket{-}) + \ket{1}(\ket{+}-\ket{-}) = \ket{0}(\ket{\emptyset} + \ket{\{x\}}) + \ket{1}(\ket{\emptyset} - \ket{\{x\}}).\] Now, let's write out what happens when running the ``attack'' described above. Start with the state of the system

    \[\sum_{a \in A^\bot}\ket{a}X^zZ^x\left(\ket{\widehat{S}} + \ket{\widehat{S}+\widehat{\Delta}}\right)\ket{0}\ket{\emptyset}\] where the second to last register is the query output register and the last register is the database register. After performing the query to $H$, we get

    \begin{align*}\sum_{a \in A^\bot}\ket{a}\bigg(&X^zZ^x\ket{\widehat{S}}\big(\ket{0}(\ket{\emptyset} + \ket{\{a,0\}}) + \ket{1}(\ket{\emptyset}-\ket{\{a,0\}})\big) \\&+ X^zZ^x\ket{\widehat{S} + \widehat{\Delta}}\big(\ket{0}(\ket{\emptyset} + \ket{\{a,1\}}) + \ket{1}(\ket{\emptyset}-\ket{\{a,1\}})\big)\bigg)\end{align*}

    Now we'll factor out the query output register since we are measuring it in the standard basis, and we'll apply Hadamard to the authenticated state.

    \begin{align*}
    &\ket{0}\sum_{a \in A^\bot}\ket{a}\bigg(X^xZ^z(\ket{S}+\ket{S+\Delta})(\ket{\emptyset} + \ket{\{a,0\}}) + X^xZ^z(\ket{S}-\ket{S+\Delta})(\ket{\emptyset} + \ket{\{a,1\}})\bigg) \\
    +&\ket{1}\sum_{a \in A^\bot}\ket{a}\bigg(X^xZ^z(\ket{S}+\ket{S+\Delta})(\ket{\emptyset} - \ket{\{a,0\}}) + X^xZ^z(\ket{S}-\ket{S+\Delta})(\ket{\emptyset} - \ket{\{a,1\}})\bigg)
    \end{align*}

    Re-writing, this is equal to 

    \begin{align*}
    &\ket{0}X^xZ^z\ket{S}\sum_{a \in A^\bot}\ket{a}(2\ket{\emptyset} + \ket{\{a,0\}} + \ket{\{a,1\}}) \\
    +&\ket{0}X^xZ^z\ket{S+\Delta}\sum_{a \in A^\bot}\ket{a}(\ket{\{a,0\}} - \ket{\{a,1\}}) \\
    +&\ket{1}X^xZ^z\ket{S}\sum_{a \in A^\bot}\ket{a}(2\ket{\emptyset} - \ket{\{a,0\}} - \ket{\{a,1\}}) \\
    +&\ket{1}X^xZ^z\ket{S+\Delta}\sum_{a \in A^\bot}\ket{a}(-\ket{\{a,0\}} + \ket{\{a,1\}}),
    \end{align*}

    and we see that the database register on the part of the state with $X^xZ^z\ket{S+\Delta}$ is supported entirely on databases that contain a vector in $A^\bot$.

    
    \item In general, we'll have to show that at \emph{any} point in which the adversary has successfully mauled their authenticated state, their $\ket{A^\bot}$ register must be entangled with the database register. Intuitively, this should be the case because the only way for the adversary to gain any (implicit) information about $\Delta$ is by querying the oracle.
\end{itemize}


\paragraph{Proof sketch.} For now we'll still take the random oracle to have one bit of output, but this should generalize to multi-bit output.

\begin{itemize}
    \item We won't need to actually compress the random oracle, but we'll imagine purifying it. Suppose we project the adversary's output onto $X^x Z^z \ket{S+\Delta}$. We want to understand what the state of the oracle registers look like. In particular, we'd like to show that if we measure the database registers in the Hadamard basis, then with overwhelming probability, we will observe a $\ket{-}$ at one of the positions $(a,b)$ for $a \in A^\bot, b \in \{0,1\}$, which means we have extracted a vector $a \in A^\bot$.
    \item We know by definition that the random oracle will never be queried on an $(a,b) \notin A^\bot \times \{0,1\}$, so it suffices to show that in the Hadamard basis, the database register has negligble amplitude on $\{\ket{+}_{a,b}\}_{a \in A^\bot,b \in \{0,1\}}$.
    \item First, we'll note that in the standard basis, the database register must have negligible amplitude on any database that is either $\ket{00}$ or $\ket{11}$ for each $a \in A^\bot$. This follows because we can imagine commuting the standard basis measurement to the beginning of the experiment, and if the adversary can output $X^xZ^z\ket{S+\Delta}$ given access to an oracle that is constant on $\ket{\widehat{S}_{\widehat{\Delta}} + z}$, then this breaks the publicly-verifiable QAS property that we proved above. Thus, there must exist some $a \in A^\bot$ such that the database is supported on only $\ket{01}$ and $\ket{10}$ in the standard basis.
    \item Next, we'll show that in the Hadamard basis, the database register has negligible amplitude on $\ket{-}\ket{-}$. Intuitively, this is because the adversary cannot simultaneously query on a vector in $\widehat{S} + z$ and $\widehat{S} + \Delta + z$. To prove this, we'll imagine measuring the authenticated state according to the random measurement oracle, and showing that the adversary cannot map to the opposite measurement result.
    \item Finally, we can show that any state with negligible amplitude on $\ket{00}$ and $\ket{11}$ in the standard basis and negligible amplitude on $\ket{-}\ket{-}$ in the Hadamard basis, must also have negligible amplitude on $\ket{+}\ket{+}$, which completes the proof.
\end{itemize}


\subsection{Protocol}

Now, we can describe the interactive protocol. Suppose for now that we just want to delegate the computation of a circuit $Q$ with classical inputs and outputs. Later, we may be able to extend to quantum inputs and outputs by using the teleport-through-encode and teleport-through-decode circuits as described by \cite{C:BroGutSte13}.

\begin{itemize}
    \item The verifier encodes the all-zeros input and all required magic states using the publicly-verifiable QAS, and sends the encoded states to the evaluator.
    \item Suppose that the circuit for $Q$ has $t$ many $T$ gates. Then the rest of the protocol will consist of $t+1$ rounds of communication. We split $Q$ up into $t+1$ parts, each part consisting of X, Z, and CNOT gates, plus standard and Hadamard basis measurements. Between each part is an application of the controlled measurement $M$ required during our implementation of the $T$ gate.
    \item Part 0: the evaluator applies the appropriate CNOT gates on authenticated data and performs standard and Hadamard basis measurements. They report their choice of input $x$ and their measurement outcomes $a_0$ to the verifier, who does the following. 
    \begin{itemize}
        \item Perform $X$ corrections on the input wires depending on $x$.
        \item Check that each measurement result does not decode to $\bot$.
        \item Determine the choice bit $c$ for the upcoming $M$ measurement.
        \item Sample $\ell_{1,0},\ell_{1,1}$, and return an oracle $O_1$ implementing $M$ as described above.
    \end{itemize} 
    \item Parts $i \in [1,\dots,t-1]$: the evaluator applies the oracle implementing $M$ and measures the output to obtain $\ell'_i$. Then they apply CNOT gates and standard and Hadamard basis measurements for the next part, and report $\ell'_i$ and their measurement outcomes $a_i$ to the verifier. The verifier does the following.
    \begin{itemize}
        \item Check that $\ell'_i \in \{\ell_{i,0},\ell_{i,1}\}$.
        \item Check that each measurement result does not decode to $\bot$ and apply appropriate one-time pad updates.
        \item Determines the choice bit $c$ for the upcoming $M$ measurement.
        \item Sample $\ell_{i+1,0},\ell_{i+1,1}$, and return an oracle $O_{i+1}$ implementing $M$ as described above.
    \end{itemize} 
    \item Part $t$: the evaluator does the same as described above. The verifier does the following.
    \begin{itemize}
        \item Check that $\ell'_t \in \{\ell_{t,0},\ell_{t,1}\}$.
        \item Check that each measurement result does not decode to $\bot$ and apply appropriate one-time pad updates.
        \item Decode the standard basis measurement on the output wires and return the output.
    \end{itemize}
\end{itemize}

\begin{align*}
    \text{\underline{Evaluator}} ~~~~~~~~~&~~~~~~~~~~~~~~~~~~~ \text{\underline{Verifier}}\\
    &\xleftarrow{\ket{\overline{\phi}}}
    \\
    &\xrightarrow{x, a_0}\\
    &\xleftarrow{O_1}\\
    &\xrightarrow{\ell'_1, a_1}\\
    &~~~~\vdots\\
    &\xleftarrow{O_t}\\
    &\xrightarrow{\ell'_t, a_t}\\
    &~~~~~~~~~~~~~~~~~ \downarrow y
\end{align*}

Here, $\ket{\overline{\phi}}$ is the initial authenticated state. For notation, let $V_0,\dots,V_t$ be the verifier next message functions, and let $\overline{V}_0,\dots,\overline{V}_t$ be the component of each next message function that checks whether the measurements results $a_i$ are valid in the sense that they don't decode to $\bot$. The rest of each $V_0,\dots,V_{t-1}$ decodes the results into bits in order to prepare $O_{i+1}$, while the rest of $V_t$ decodes the results into bits in order to determine the output $y$.


\subsection{Security}

What can we prove about this protocol? For now, let's suppose that $Q$ is pseudo-deterministic. We will want to prove security guarantees in the case where the evaluator gets some sort of oracle access to the verifier next-message functions.

\paragraph{Step 1: No $T$ gates, oracle access to verifier.} Suppose that the circuit is a Clifford circuit, so the protocol is non-interactive, but the evaluator gets oracle access to the single verifier functionality $V_0$. Obfuscating a pseudo-deterministic Clifford circuit in this way is silly because such circuits can only implement a classical function. However, it could still be useful to analyze.

Note that $V_0$ can be implemented by first decoding all the measurement results and then applying a classical function on $x$ and the resulting bits. Consider the state the adversary submits for its first $V_0$ query. By the publicly-verifiable QAS (\cref{claim:QAS}), this state is either rejected by the QAS verifier, or it is an encoding of the honest output state. Thus, $V_0$ can be simulated just given the accept projector for the QAS scheme and an oracle for the functionality $Q$, and the adversary can never make $V_0$ output a invalid output.
    
    
    
    
    


\paragraph{Step 2: One $T$ gate.} Now, suppose that we add one $T$ gate to the circuit, and for now suppose that the adversary gets oracle access to the final verification function but only one-time access to the intermediate verification function that outputs the $M$-measurement oracle.

First, we can try to prove a claim specifically about the $M$-measurement oracle. Intuitively, we want to show that the oracle for $M$ ``forces'' a measurement of $M$ on authenticated qubits.

\begin{itemize}
    \item This is a simplified setting, but will at least be necessary to show. Suppose the adversary is given a two-qubit authenticated state \[X^{x_1}Z^{z_1} \otimes X^{x_2}Z^{z_2}\left(\alpha_{00}\ket{S}\ket{S} + \alpha_{01}\ket{S}\ket{S+\Delta} + \alpha_{10}\ket{S+\Delta}\ket{S} + \alpha_{11}\ket{S+\Delta}\ket{S+\Delta}\right)\] along with the oracle \begin{align*}&(S+x_1,S+x_2),(S+\Delta + x_1,S+\Delta+x_2) \to \ell_0\\&(S+x_1,S+\Delta+x_2),(S+ x_1,S+\Delta+x_2) \to \ell_1.\end{align*} We want to claim that the adversary cannot tell if the underlying authenticated state was pre-measured in the $\{\ketbra{00}{00} + \ketbra{11}{11}, \ketbra{01}{01} + \ketbra{10}{10}\}$ basis.
    \item By mapping-distinguishing (actually we'll need some version of this that works with privately verifiable predicates), it suffices to show that given the result of this measurement, say \[X^{x_1}Z^{z_1} \otimes X^{x_2}Z^{z_2}(\alpha_0\ket{S}\ket{S} + \alpha_1\ket{S+\Delta}\ket{S+\Delta}),\] along with the oracle, the adversary cannot output a vector in $(S+x_1,S+\Delta+x_2)$ or $(S+\Delta+x_1,S+x_2)$.
    \item We can first switch the oracle to change how it answers on $(S+x_1,S+\Delta+x_2),(S+\Delta+x_1,S+x_2)$ from $\ell_1$ to $\ell_0$. If the adversary notices this difference, it could have anyway won the game without the query. Now, the oracle is essentially just a verifiction oracle for the authentication scheme in the standard basis, that is, it accepts on $S_\Delta + x_1, S_\Delta + x_2$.
    \item Now, sample a random superspace $T \supset S_\Delta$ and let the oracle accept on $T+x_1, T+x_2$. 
    \item At this point, we can use the same ideas as in the proof of \cref{claim:QAS}. We use the Pauli twirl inside $T$ to show that the adversary can only apply a mixture over linear shifts. By the randomness of $S,\Delta$, this will fail to produce a vector in $(S+x_1,S+\Delta+x_2),(S+\Delta+x_1,S+x_2)$ except with negligible probability.
\end{itemize}

In the actual protocol, the adversary can also query the final verifier, who either aborts or decodes the final output of the computation. So, we will have to show this mapping-distinguishing claim even when the adversary has oracle access to this function. Intuitively, this shouldn't be an issue. By Step 1, the adversary can only make this oracle accept and output the correct output of the computation, or reject (this claim also uses the randomness of $\ell_1$, since it relies on the adversary not being able to guess the ``wrong'' output $\ell_1$ given only access to $\ell_0$.). Thus, it can be simulated by a public-verification oracle for the QAS. The arguments above should be valid in the presence of such an oracle, again using the ideas from \cref{claim:QAS}.





\subsection{Compiling to obfuscation}

We construct an obfuscation candidate from the above interactive scheme. Let $U$ be the universal circuit and suppose we want to obfuscate a psuedo-deterministic circuit $Q$. The obfuscation will consist of \[\ket{\overline{\phi_Q}},\ket{\sk},C[V_0],\dots,C[V_t],\] where $\ket{\phi_Q}$ is the description of the state input to $U$ that implements $Q$ on the all-zeros input, $\ket{\sk}$ is the secret key for a signature token scheme, and $C[V_0],\dots,C[V_t]$ are classical oracles constructed based on the verifier next message functions $V_0,\dots,V_t$. 

\begin{itemize}
    \item The signature token is used to sign the evaluator's choice of input $x$. This will be used to ensure that the evaluator cannot change its input in the middle of its interaction with the oracles.
    \item Each oracle $C[V_i]$ takes as input the entire transcript produced so far, including $x$, the signature $\sigma_x$, measurement results $a_0,\dots,a_i$, and output labels  $\ell'_1,\dots,\ell'_i$ from the $M$ measurements. It applies a random oracle to the transcript in order to sample $\ell_{i+1,0},\ell_{i+1,1}$, and then implements $O_{i+1}$. That is, for $i \in [0,t-1]$,
    \[C[V_i] : (x,\sigma_x,a_0,\ell'_1,a_1,\dots,\ell'_i,a_i,s_1,s_2) \to \{\ell_{i+1,0},\ell_{i+1,1},\bot\},\] and \[C[V_t] : (x,\sigma_x,a_0,\ell'_1,a_1,\dots,\ell'_t,a_t) \to \{y,\bot\}.\]
\end{itemize}



For the next lemma, we set up some notation. Consider a quantum operation $U^H$ with access to a random oracle $H$ sampled as a uniformly random function from $\{0,1\} \times \{0,1\}^{p_1} \to \{0,1\}^{p_2}$. For each $z \in \{0,1\}^{p_2}$, define the following states:
\[\ket{\phi_z} \coloneqq \frac{1}{\sqrt{2^{p_2}}}\sum_{y \in \{0,1\}^{p_2}}(-1)^{y \cdot z}\ket{y}, ~~~~~~ \ket{\Phi_z} \coloneqq \frac{1}{\sqrt{2^{p_2}}}\sum_{y \in \{0,1\}^{p_2}}(-1)^{y \cdot z}\ket{y}\ket{y},\] and let \[\ket{\phi} \coloneqq \ket{\phi_{0^{p_2}}}, ~~~~~~ \ket{\Phi} \coloneqq \ket{\Phi_{0^{p_2}}}.\]

We will introduce a ''database register'' that stores the description of $H$, and implement each query that $U$ makes as a unitary that operates on $U$'s workspace and the database register. Furthermore, we will purify the sampling of $H$, and initialize the database register to the state \[\ket{+_H} \coloneqq \frac{1}{\sqrt{(2p_1)2^{p_2}}}\sum_{H}\ket{H} = \ket{\phi}^{\otimes 2p_1}.\] Next, define the projector (that is digaonal in the standard basis) \[\Pi_{\mathsf{const}} \coloneqq \sum_{H : H(0,x)=H(1,x) \forall x \in \{0,1\}^{p_1}} \ketbra{H}{H}\] and the projector (that is diagonal in the Hadamard basis) \[\Pi_{\mathsf{double}} \coloneqq \sum_{x \in \{0,1\}^{p_1}}(\bbI-\ketbra{\phi}{\phi})_{0,x} \otimes (\bbI-\ketbra{\phi}{\phi})_{1,x} \otimes \bbI_{(b,x'): x' \neq x}.\]

\begin{lemma}\label{lemma:extraction}
    Let $H$ be a random oracle sampled as a uniformly random function from $\{0,1\} \times \{0,1\}^{p_1} \to \{0,1\}^{p_2}$, and let $\{U_k,\ket{\psi_k},\Pi_k\}_{k \in \cK}$ be a set of random oracle aided unitaries $U_k$, states $\ket{\psi_k}$, and projective measurements $\Pi_k$ on the workspace of $U_k$. Suppose that there exists an $\epsilon$ such that \[\E_k\left[\big\|(\Pi_{\mathsf{const}} \otimes \Pi_k)U_k(\ket{+_H} \otimes \ket{\psi_k}) \big\|^2\right] \leq \epsilon,\] and \[\E_k\left[\big\| (\Pi_{\mathsf{double}} \otimes \bbI)U_k(\ket{+_H} \otimes \ket{\psi_k})\big\|^2\right] \leq \epsilon.\] Then,
    \[\E_k\left[\big\|(\ketbra{+_H}{+_H} \otimes \Pi_k)U_k(\ket{+_H} \otimes \ket{\psi_k}) \big\|^2\right] \leq 3\sqrt{\epsilon}p_1 2^{p_2}.\]
\end{lemma}

\begin{proof} ()
    Define \[\ket{\psi'_k} \coloneqq (\bbI \otimes \Pi_k)U_k(\ket{+_H} \otimes \ket{\psi_k}),\] 
    
    and write 

    \[\ket{\psi'_k} = \ketbra{+_H}{+_H}\ket{\psi'_k} + (\bbI - \Pi_{\mathsf{double}}-\ketbra{+_H}{+_H})\ket{\psi'_k} + \Pi_{\mathsf{double}}\ket{\psi'_k} \coloneqq \ket{\psi'_{k,0}} + \ket{\psi'_{k,1}} + \ket{\psi'_{k,2}}.\]

    Observe that \[\Pi_{\mathsf{const}}\ket{\psi'_{k,0}} = \frac{\|\ket{\psi'_{k,0}}\|}{\sqrt{p_1 2^{p_2}}}\ket{\Phi}^{\otimes p_1},\] and \[\Pi_{\mathsf{const}}\ket{\psi'_{k,1}} \in \bigotimes_{x \in \{0,1\}^{p_1}}\mathsf{span}\left\{\ket{\Phi_z}_x\right\}_{z \in \{0,1\}^{p_2} \setminus \{0^{p_2}\}}.\]

    By the first and second conditions, we have that \[\E_k\left[
    \|\Pi_{\mathsf{const}}\ket{\psi'_{k}}\|^2\right] \leq \epsilon, ~~ \text{and} ~~ \E_k\left[\|\ket{\psi'_{k,2}}\|^2\right] \leq \epsilon.\]  Thus, using the fact that $\ket{\Phi}$ is orthogonal to $\ket{\Phi_z}$ for all $z \neq 0^{p_2}$, we have that \[\epsilon \geq \E_k\left[\|\Pi_{\mathsf{const}}\ket{\psi'_k}\|^2\right] \geq \E_k\left[\|\Pi_{\mathsf{const}}\ket{\psi'_{k,0}}\|^2\right] - 2\sqrt{\epsilon} = \frac{1}{p_1 2^{p_2}}\E_k\left[\|\ket{\psi'_{k,0}}\|^2\right] - 2\sqrt{\epsilon},\] and so \[\E_k\left[\|\ket{\psi'_{k,0}}\|^2\right] \leq 3\sqrt{\epsilon}p_1 2^{p_2},\] which completes the proof of the claim.
    
    
    
    
    
\end{proof}


 Consider a slightly modified distribution $O'$ that samples the labels $\ell$ using two nested random oracles.\\

\noindent\underline{$O'(1^\secp,x^*,\ket{\psi})$}
\begin{itemize}
    \item Sample $k = (S,\Delta,\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}) \gets \Gen(n,m)$, compute $\ket{\widetilde{\psi}} = \Enc_k\ket{\psi}$, and let $V_k$ be the public verification oracle for the authentication scheme.
    \item For each $w \in \cW$, derive $x_w,z_w$ from $\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}$ and the circuit topology using the CNOT update rule $(x_1,z_1),(x_2,z_2) \to (x_1,z_1 \oplus z_2),(x_1 \oplus x_2,z_2)$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample random oracles $H_1 : \{0,1\} \times \{0,1\}^{\log(m')\kappa + \log(t)} \to \{0,1\}^{3(\log(m')\kappa + \log(t) + 1)}$ and $H_2 : \{0,1\}^* \to \{0,1\}^\zeta$. For any $i \in [t]$ and string $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i)$, define two labels indexed by a bit $b\in\{0,1\}$: 
    \[ \ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i} \coloneqq H_2(H_1(b,(x,\sigma_x,i)),\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i).\]
    \item For each $i \in [t]$, let $F_i[x^*]$ be identical to $F_i$ (\proref{fig:F-oracle}) except that it aborts on any input that begins with $x^*$.
    \item Output \[\ket{\widetilde{\psi}},\ket{\sk},V_k,F_1[x^*],\dots,F_t[x^*].\]
\end{itemize}

Note that these distributions are identical conditioned on $H_1$ being injective, which happens with $1-\negl(\kappa)$ probability, so it suffices to prove the lemma when instantiated with $O'$ instead of $O$. Next, we will purify $H_1$. Moreover, anytime that $F_2[x^*],\dots,F_t[x^*]$ is about to query $H_1$ during a \textbf{Decode $\{\ell_\iota\}_\iota$} step, we will first check to see if the database has been initialized at the input yet, and if not we will not perform the query. Since these queries are all comparison queries, this will only introduce a $\negl(\kappa)$ trace distance in the experiment. This will ensure that $H_1$ indices will only be initialized during the actual measurement step, and will be necessary for proving \cref{lemma:doub}.

Now, we will show that conditioned on $\Pi[\Sigma_{\vk,x^*}] \otimes \Pi\left[\widetilde{P}_{k,A,\theta}\right]$ accepting, there is a good probability (close to 1) that when we measure the database register of $H_1$ in the Hadamard basis, we extract an input $(b,x,\sigma_x,i)$ which in particular gives us a valid signature on some $x \neq x^*$. This means that if the expectation in the lemma statement is $1/\poly(\kappa)$, a reduction can obtain signatures on two different messages with probability $1/\poly(\kappa)$, which is a contradiction.

To show this, we combine \cref{lemma:extraction} with the following two lemmas \cref{lemma:const} and \cref{lemma:doub}, which shows that the probability of measuring $\ket{+_H}$ in the database register conditioned on $\Pi[\Sigma_{\vk,x^*}] \otimes \Pi\left[\widetilde{P}_{k,A,\theta}\right]$ accepting is $\negl(\kappa)$, and thus some input must be observed with very high probability.


\end{proof}

\begin{lemma}\label{lemma:const}
    For any $x^*$, state $\ket{\psi}$, BB84 state projector $\Pi_{A,\theta}$ such that $\Pi_{A,\theta}\ket{\psi} = 0$, and unitary $U$ with $\poly(\secp)$ oracle queries, it holds that
    \[\E_{\left(\ket{\widetilde{\psi}},\ket{\sk},V_k,F_1[x^*],\dots,F_t[x^*]\right) \gets O'(1^\secp,x^*,\ket{\psi})}\left[\big\| \left(\Pi_{\mathsf{const}} \otimes \Pi\left[\widetilde{P}_{k,A,\theta}\right]\right)U^{V_k,F_1[x^*],\dots,F_t[x^*]}\ket{\widetilde{\psi}}\ket{\sk}\ket{+_{H_1}}\big\|^2\right] \leq \negl(n).\] 
\end{lemma}

\begin{proof}
%
\end{proof}

\begin{lemma}\label{lemma:doub}
    For any $x^*$, state $\ket{\psi}$, and unitary $U$ with $\poly(\secp)$ oracle queries, it holds that
    \[\E_{\left(\ket{\widetilde{\psi}},\ket{\sk},V_k,F_1[x^*],\dots,F_t[x^*]\right) \gets O'(1^\secp,x^*,\ket{\psi})}\left[\big\| \Pi_{\mathsf{doub}} U^{V_k,F_1[x^*],\dots,F_t[x^*]}\ket{\widetilde{\psi}}\ket{\sk}\ket{+_{H_1}}\big\|^2\right] \leq 2^{2t} \cdot \negl(n).\] 
\end{lemma}

\begin{proof}
    %
\end{proof}



Suppose that for some $\tau \in [t]$, we perform the first $\tau$ measurement layers on $\ket{\psi}$ with input $x^*$ to obtain $\overline{a}_1,r_1,\dots,\overline{a}_\tau,r_\tau$, and let $\ket{\psi_{x^*,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}}}$ be the measured state. We define a partially simulated obfuscation as follows.\\

\noindent\underline{$\ParSim\left(1^\secp,x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]},\ket{\psi_{x^*,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}}}\right)$}

\begin{itemize}
    \item Sample $k = (S,\Delta,\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}) \gets \Gen(n,m)$ and compute $\ket{\widetilde{\psi}} = \Enc_k\ket{\psi_{x^*,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}}}$. 
    \item For each $w \in \cW$, derive $x_w,z_w$ from $\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}$ and the circuit topology using the CNOT update rule $(x_1,z_1),(x_2,z_2) \to (x_1,z_1 \oplus z_2),(x_1 \oplus x_2,z_2)$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\zeta$. For any $i \in [t]$ and string $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i)$, define two labels indexed by a bit $b\in\{0,1\}$: 
    \[ \ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i} \coloneqq H(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,b).\]
    \item For each $i \in [1,\dots,\tau]$, prepare an oracle $F^\Sim_i[x^*,\{r_\iota\}_{\iota \in [i]}]$ that implements the classical functionality described in \proref{fig:F-sim-i}.

\protocol{$F^\Sim_i[x^*,\{r_\iota\}_{\iota \in [i]}]$ Functionality}{$F^\Sim_i[x^*,\{r_\iota\}_{\iota \in [i]}]$}{fig:F-sim-i}{

\begin{itemize}
    \item \textbf{Input:} $\left(x,\sigma_{x},\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s_{i,0}^M,s_{i,1}^M\right)$. \item \textbf{Branch on $x$:} If $x \neq x^*$, then output $F_i\left(x,\sigma_{x},\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s_{i,0}^M,s_{i,1}^M\right)$. Otherwise, continue.
    \item \textbf{Check token:} Check that $\TokVer(\vk,x,\sigma_x) = \top$, and abort and output $\bot$ if not.
    \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [i]}$:} For each $\iota \in [i]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_\iota \union \cW^H_\iota}$. For each $w \in \cW^S_\iota$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
    \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [i-1]}$:} For each $\iota \in [i-1]$, output $\bot$ if $\ell_\iota \neq \ell^{r_\iota}_{\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$. Otherwise, continue.
    \item \textbf{Compute next label:} Parse $\cW_i^M = \{w_0,w_1\}$. If $(s^M_{i,0},s^M_{i,1}) \notin \{(S_\Delta + x_{w_0}, S_\Delta + x_{w_1})\}$, output $\bot$. Otherwise, continue with $\ell_i = \ell^{r_i}_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i}$.
        \item \textbf{Output:} $\ell_i$.
\end{itemize}

}

    \item For each $i \in [\tau+1,\dots,t]$, prepare an oracle $F_i^\ParSim[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$ that implements the classical functionality described in \proref{fig:F-parsim-i}.

\protocol{$F_i^\ParSim[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$ Functionality}{$F_i^\ParSim[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$}{fig:F-parsim-i}{

    \begin{itemize}
        \item \textbf{Input:} $\left(x,\sigma_{x},\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s_{i,0}^M,s_{i,1}^M\right)$. \item \textbf{Branch on $x$:} If $x \neq x^*$, then output $F_i\left(x,\sigma_{x},\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s_{i,0}^M,s_{i,1}^M\right)$. Otherwise, continue. 
        \item \textbf{Check token:} Check that $\TokVer(\vk,x,\sigma_x) = \top$, and abort and output $\bot$ if not.
        \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [\tau]}$:} For each $\iota \in [\tau]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_\iota \union \cW^H_\iota}$. For each $w \in \cW^S_\iota$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
        \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [\tau]}$:} For each $\iota \in [\tau]$, output $\bot$ if $\ell_\iota \neq \ell^{r_\iota}_{\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$. Otherwise, continue. 
        \item \textbf{Decode $\{\overline{s}_\iota\}_{\iota \in [\tau+1,\dots,i]}$:} For each $\iota \in [\tau+1,\dots,i]$, $\overline{s}_\iota = \{s_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ is a set of vectors that are supposed to be standard or Hadamard basis measurements of authenticated wires. For $w \in \cW^S_\iota$, define 
        
        \[a_w = \begin{cases} 0 \text{ if } s_w \in S+x_w\\ 1 \text{ if } s_w \in S+\Delta+x_w \\ \bot \text{ else}
        \end{cases},\]

         and for $w \in \cW^H_\iota$, define 

         \[a_w = \begin{cases} 0 \text{ if } s_w \in \widehat{S}+z_w\\ 1 \text{ if } s_w \in \widehat{S}+\widehat{\Delta}+z_w \\ \bot \text{ else}
        \end{cases},\]
        
        If any were $\bot$, abort and output $\bot$. Otherwise, define $\overline{a}_\iota = \{a_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ for each $\iota \in [\tau+1,\dots,i]$.
        \item \textbf{Decode $\{\ell_\iota\}_{\iota \in [\tau+1,i-1]}$:} For each $\iota \in [\tau+1,i-1]$, define the bit $r_\iota=b$ if $\ell_\iota = \ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$, and otherwise abort and output $\bot$.
        \item \textbf{Compute next control bit:} Compute $c_i = f_i(x,\overline{a}_1,r_1,\dots,\overline{a}_{i-1},r_{i-1},\overline{a}_i)$.
        \item \textbf{Compute next label:} For $b \in \{0,1\}$, define $\ell^b_i =\ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i}$, and parse $\cW_i^M = \{w_0,w_1\}$. If $c_i = 0$, define

        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\} \\
            \bot \text{ else}
        \end{cases},\]

        and if $c_i = 1$, define
        
        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\} \\ 
            \bot \text{ else}
        \end{cases}.\]

        \item \textbf{Output:} $\ell_i$
    \end{itemize}

    }

    \item Prepare an oracle $G^{\ParSim}[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$ that implements the classical functionality described in \proref{fig:G-parsim}.

\protocol{$G^{\ParSim}[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$ Functionality}{$G^{\ParSim}[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]$}{fig:G-parsim}{

    \item \textbf{Input:} $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{t},\ell_{t},\overline{s}_{t+1})$.
    \item \textbf{Branch on $x$:} If $x \neq x^*$, then output $G^\Sim[Q]\left(x,\sigma_{x},\overline{s}_1,\ell_1,\dots,\overline{s}_{t},\ell_{t},\overline{s}_{t+1}\right)$. Otherwise, continue. 
    \item \textbf{Check token:} Check that $\TokVer(\vk,x,\sigma_x) = \top$, and abort and output $\bot$ if not.
    \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [\tau]}$:} For each $\iota \in [\tau]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_\iota \union \cW^H_\iota}$. For each $w \in \cW^S_\iota$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
    \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [\tau]}$:} For each $\iota \in [\tau]$, output $\bot$ if $\ell_\iota \neq \ell^{r_\iota}_{\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$. Otherwise, continue. 
    \item \textbf{Decode $\{\overline{s}_\iota\}_{\iota \in [\tau+1,\dots,t+1]}$:} For each $\iota \in [\tau+1,\dots,t+1]$, $\overline{s}_\iota = \{s_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ is a set of vectors that are supposed to be standard or Hadamard basis measurements of authenticated wires. For $w \in \cW^S_\iota$, define 
        
        \[a_w = \begin{cases} 0 \text{ if } s_w \in S+x_w\\ 1 \text{ if } s_w \in S+\Delta+x_w \\ \bot \text{ else}
        \end{cases},\]

         and for $w \in \cW^H_\iota$, define 

         \[a_w = \begin{cases} 0 \text{ if } s_w \in \widehat{S}+z_w\\ 1 \text{ if } s_w \in \widehat{S}+\widehat{\Delta}+z_w \\ \bot \text{ else}
        \end{cases},\]
        
        If any were $\bot$, abort and output $\bot$. Otherwise, define $\overline{a}_\iota = \{a_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ for each $\iota \in [\tau+1,\dots,t+1]$.
        \item \textbf{Decode $\{\ell_\iota\}_{\iota \in [\tau+1,\dots,t]}$:} For each $\iota \in [\tau+1,\dots,t]$, define the bit $r_\iota=b$ if $\ell_\iota = \ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$, and otherwise abort and output $\bot$.
        \item \textbf{Compute output:} Compute $y = g(x,\overline{a}_1,r_1,\dots,\overline{a}_t,r_t,\overline{a}_{t+1})$.
        \item \textbf{Output:} $y$
}

    \item Output the partially simulated obfuscated circuit 

    \[\ket{\widetilde{\psi}},\ket{\sk},O^\ParSim_\tau,\] where
    
    
    
    \[O^\ParSim_\tau \coloneqq \left\{F_i^\Sim[x^*,\{r_\iota\}_{\iota \in [i]}]\right\}_{i \in [\tau]}, \left\{F_i^\ParSim[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}]\right\}_{i \in [\tau+1,\dots,t]},G^\ParSim[x^*,\tau,\{\overline{a}_\iota,r_\iota\}_{\iota \in [\tau]}].\]

    
\end{itemize}


\protocol{$G^\Sim[Q]$ Functionality}{$G^\Sim[Q]$}{fig:G-sim-y}{
    \begin{itemize}
        \item \textbf{Input:} $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{t-1},\ell_t,\overline{s}_{t+1})$.
        \item \textbf{Check token:} Check that $\TokVer(\vk,x,\sigma_x) = \top$, and abort and output $\bot$ if not.
        \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [t+1]}$}: For each $i \in [t]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_i \union \cW^H_i}$. For each $w \in \cW^S_i$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
        \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [t]}$}: For each $i \in [t]$, output $\bot$ if $\ell_i \neq \{\ell^0_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i},\ell^1_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i}\}$. Otherwise, continue.
        \item \textbf{Output:} $Q(x)$.
    \end{itemize}

}


\noindent\underline{$\Punc(1^\secp,Q,x^*,\ket{\psi})$}
\begin{itemize}
    \item Sample $k = (S,\Delta,\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}) \gets \Gen(n,m)$, compute $\ket{\widetilde{\psi}} = \Enc_k\ket{\psi}$, and let $V_k$ be the public verification oracle for the authentication scheme.
    \item For each $w \in \cW$, derive $x_w,z_w$ from $\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}$ and the circuit topology using the CNOT update rule $(x_1,z_1),(x_2,z_2) \to (x_1,z_1 \oplus z_2),(x_1 \oplus x_2,z_2)$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\zeta$. For any $i \in [t]$ and string $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i)$, define two labels indexed by a bit $b\in\{0,1\}$: 
    \[ \ell^b_{x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i} \coloneqq H(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,b).\]
    \item For each $i \in [t]$, let $F_i[x^*]$ be identical to $F_i$ (\proref{fig:F-oracle}) except that it aborts on any input that begins with $x^*$. Let $G[Q,x^*]$ be identical to $G^\Sim[Q]$ except that it aborts on any input that begins with $x^*$.
    \item Output \[\ket{\widetilde{\psi}},\ket{\sk},V_k,O_\Punc[x^*],\]
    
    where \[O^\Punc[x^*] = F_1[x^*],\dots,F_t[x^*],G[Q,x^*].\]
\end{itemize}


\begin{itemize}

    
    \item \textbf{Public-verification oracle:} Given an authentication key $k = (S,\Delta,\{x_i,z_i\}_{i \in [m]})$, define the classical function $V_k(b,L,s) \to \{\top,\bot\}$ as follows.
    \begin{itemize}
        \item Take as input a bit $b \in \{0,1\}$, a subset $L \subseteq [m]$, and a vector $s \in \bbF_2^{2n+1}$.
        \item If $b=0$, output $\top$ if $s \in S_\Delta + \sum_{i \in L} x_i$, and otherwise output $\bot$.
        \item If $b=1$, output $\top$ if $s \in \widehat{S}_{\widehat{\Delta}} + \sum_{i \in L} z_i$, and otherwise output $\bot$.
    \end{itemize}
    
    

    \item \textbf{BB84 state projectors:} Given a string $a \in \{0,1\}^m$ and a subset $\theta \subseteq [m]$, define the projector \[\Pi_{a,\theta} \coloneqq \bigotimes_{i \in \theta}\ketbra{a_i}{a_i} \bigotimes_{i \notin \theta} H\ketbra{a_i}{a_i}H,\] and given a set $A$ of strings $a$, define the ``BB84 state projector'' \[\Pi_{A,\theta} \coloneqq \sum_{a \in A} \Pi_{a,\theta}.\]

    Next, given an authentication key $k = (S,\Delta,\{x_i,z_i\}_{i \in [m]})$ along with the description of a BB84 state projector $(A,\theta)$, define the set \[\widetilde{P}_{k,A,\theta} \coloneqq \bigcup_{a \in A}\left(\bigotimes_{i \in \theta}(S+a_i\cdot \Delta + x_i) \bigotimes_{i \notin \theta}(\widehat{S}+a_i \cdot \widehat{\Delta} + z_i)\right),\]

    where in this context, $\bigotimes$ is a cartesian product of sets.
    
    
    
    


    
\end{itemize}

Suppose we give an adversary (i) an encoded state $\Enc_k\ket{\psi}$, where $\ket{\psi}$ is in the kernel of some BB84 state projector $\Pi_{A,\theta}$, and (ii) access to classical oracles that check for membership in the affine subspaces that define the authentication scheme (note that this is potentially more powerful than a quantum oracle that projects onto the codespace). Intuitively, we want to show that the adversary cannot maul the encoding of $\ket{\psi}$ to the encoding of $\ket{\psi'}$ for some $\ket{\psi'} \in \mathsf{im}(\Pi_{A,\theta})$. However, we will ask for something stronger: we will want to show that the adversary cannot output \emph{any} vector in the support of $\Enc_k\ket{\psi'}$ for some $\ket{\psi'} \in \mathsf{Im}(\Pi_{A,\theta})$. We can capture this by projecting their output onto $\Pi[\widetilde{P}_{k,A,\theta}]$. Note that it is meaningful to talk about the support of an authenticated state for states that are collapsed in the standard or Hadamard basis, since in this case the support is just the affine subspace that defines the authenticated $\ket{0},\ket{1},\ket{+},$ or $\ket{-}$ state. This is why we restrict to BB84 state projectors, which will be sufficient for reasoning about the obfuscation scheme.


\begin{theorem}\label{thm:basic-authentication}
The scheme satisfies the security definition.
\end{theorem}

\begin{proof}
    Outline: 
    \begin{itemize}
        \item Sample random superspaces $T \supset S_\Delta$ and $R \supset \widehat{S}_{\widehat{\Delta}}$ of dimension $3n/2 + 1$, and give the adversary oracle access to $V_{k,T,R}$, which is defined like $V_k$ except that $T$ is used in place of $S_\Delta$ and $R$ is used in place of $\widehat{S}_{\widehat{\Delta}}$.
        
        
        
        \item Fix a choice of $R^\bot \subset T$, where $R$ has dimension $n/2$ and $T$ has dimension $3n/2 + 1$, and let $\co(T),\co(R)$ be sets of coset representatives of $T$ and $R$. We can then sample $S,\Delta$ uniformly at random such that $R^\bot \subset S \subset S_\Delta \subset T$, and sample each $x_i,z_i$ in two parts: $x_i = x_{i,T} + x_{i,\co(T)}$ and $z_i = z_{i,R} + z_{i,\co(R)}$, where $x_{i,T} \gets T$ and $x_{i,\co(T)} \gets \co(T)$ (and analogously for $z_i$).
        \item We give out $(T,R,x_{1,\co(T)},z_{1,\co(R)},\dots,x_{m,\co(T)},z_{m,\co(R)})$ in the clear so that the adversary can implement $V_{k,T,R}$ by itself. We apply the Pauli twirl within the space defined by $T,R$ using the randomness of $x_{i,T}$ and $z_{i,R}$ to reduce the adversary's attack to a mixture over fixed Pauli attacks $X^x Z^z$ for $x \in T,z \in R$.
        \item Let $\theta$ be the set that defines the bases of the BB84 projector. For any fixed non-zero Pauli attack $(x,z)$, there are two cases: (1) there exists an $i \in \theta$ such that $x_i \neq 0^n$ or an $i \notin \theta$ such that $z_i \neq 0^n$, in which case the randomness of $S,\Delta$ can be used to show that the attack will bring the state outside of the support of $\Pi[\widetilde{P}_{k,A,\theta}]$, or (2) $x_i = 0^n$ for all $i \in \theta$ and $z_i = 0^n$ for all $i \notin \theta$, in which case this attack cannot bring a state outside of $\Pi[\widetilde{P}_{k,A,\theta}]$ into $\Pi[\widetilde{P}_{k,A,\theta}]$.
    \end{itemize}
\end{proof}


\begin{corollary}\label{cor:basic-authentication}
Let $n(\secp),m(\secp) = \poly(\secp)$. For any $m$-qubit state $\ket{\psi}$, any BB84 state projector $\Pi_{A,\theta}$ such $\Pi_{A,\theta}\ket{\psi} = 0$, and any unitary $U$ with $\poly(\secp)$ oracle queries,\[\E_{k \gets \Gen(n,m)}\left[\big\|\Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{V_k}\Enc_k\ket{\psi} \big\|^2\right] = \negl(\secp).\]
\end{corollary}



\begin{definition}[Quantum State Obfuscation]\label{def:obf}
    Let $\{\ket{\psi_\secp},C_\secp\}_{\secp \in \bbN}$ be a family of (pseudo)-deterministic quantum implementations (\cref{def:quantum-imp}) with induced maps $\{Q_\secp\}_{\secp \in \bbN}$. A quantum state obfuscator is a pair of QPT algorithms $(\QObf,\QEval)$ with the following syntax.
    \begin{itemize}
        \item $\QObf(1^\secp,\ket{\psi},C) \to \ket{\widetilde{\psi}}$: The obfuscator takes as input the security parameter $1^\secp$ and a quantum implementation $(\ket{\psi},C)$, and outputs an obfuscated state $\ket{\widetilde{\psi}}$.
        \item $\QEval(x,\ket{\widetilde{\psi}}) \to y$: The evaluation algorithm takes an input $x \in \{0,1\}^{m_{\mathsf{in}}}$ and an obfuscated state $\ket{\widetilde{\psi}}$, and outputs $y \in \{0,1\}^{m_{\mathsf{out}}}$.
    \end{itemize}
    \textbf{Correctness} is defined as follows.
    \[\forall x \in \{0,1\}^{m_{\mathsf{in}}}, \Pr\left[\QEval\left(x,\ket{\widetilde{\psi}}\right) = Q_\secp(x) : \ket{\widetilde{\psi}} \gets \QObf\left(1^\secp,\ket{\psi_\secp},C_\secp\right)\right] = 1-\negl(\secp).\]
    We define two notions of security.
    \begin{itemize}
        \item \textbf{Virtual Black-Box Obfusation}: For any QPT adversary $\{A_\secp\}_{\secp \in \bbN}$, there exists a QPT simulator $\{\Sim_\secp\}_{\secp \in \bbN}$ such that for any family of deterministic quantum implementations $\{\ket{\psi_\secp},C_\secp\}_{\secp \in \bbN}$ with induced maps $\{Q_\secp\}_{\secp \in \bbN}$, \[\bigg|\Pr\left[1 \gets A_\secp(\QObf(1^\secp,\ket{\psi_\secp},C_\secp))\right] - \Pr\left[1 \gets \Sim_\secp^{Q_\secp}\right]\bigg| = \negl(\secp).\]
        %
        \item \textbf{Indistinguishability Obfuscation}: For any pair of families of deterministic quantum implementations $\{\ket{\psi_{\secp,0}},C_{\secp,0}\}_{\secp \in \bbN}, \{\ket{\psi_{\secp,1}},C_{\secp,1}\}_{\secp \in \bbN}$ with the same induced map $\{Q_\secp\}_{\secp \in \bbN}$, and any QPT adversary $\{A_\secp\}_{\secp \in \bbN}$,
        \[\bigg|\Pr\left[1 \gets A_\secp(\QObf(1^\secp,\ket{\psi_{\secp,0}},C_{\secp,0}))\right] - \Pr\left[1 \gets A_\secp(\QObf(1^\secp,\ket{\psi_{\secp,1}},C_{\secp,1})\right]\bigg| = \negl(\secp).\]
    \end{itemize}
\end{definition}

\begin{remark}[Classical Oracle Model]
In this work, we construct quantum state obfusation in the \emph{classical oracle model}. In this model, we allow $\QObf$ to additionally output the description of a classical deterministic functionality $O$, and both $\QEval$ and the adversary $A_\secp$ are granted quantum-accessible oracle access to $O$. Any scheme in the classical oracle model may be heuristically instantiated in the plain model by using a post-quantum indistinguishability obfuscator to obfuscate $O$ and include its obfuscation in the description of the state $\ket{\widetilde{\psi}}$.
\end{remark}

==> obfuscator-old.tex <==
\section{Obfuscation Construction}


Consider any classical input/output deterministic  quantum circuit, and write it using the representation described above:

\[\ket{\psi},C_1,f_1,C_2,\dots,f_t,C_{t+1},g,\] where $\ket{\psi}$ includes all of the required magic states, ancillary 0 states, and an input register initialized to 0. Define $\cW,\cW^{\mathsf{in}},\{\cW_i^S,\cW_i^H,\cW_i^M\}_{i \in [t]},\cW^{\mathsf{out}}$ as above, and $m \coloneqq |\cW^{\mathsf{in}}|$. We will consider $C_1,f_1,C_2,\dots,f_t,C_{t+1},g$ to be public, and the goal of the obfuscation is to hide $\ket{\psi}$. The construction is given in \proref{fig:qobf}.

\protocol{$\QObf$}{Quantum obfuscation construction}{fig:qobf}{

\noindent Public parameters: 
    \begin{itemize}
        \item Security parameter $\secp$.
        \item Circuit topology $C_1,f_1,\dots,C_t,f_t,C_{t+1},g,\cW$, with $m = |\cW_{\mathsf{in}}|$.
        \item $n = \poly(\secp,m,t)$. %
    \end{itemize}

\noindent $\QObf(1^\secp,\ket{\psi})$: 

\begin{itemize}
    \item Sample $k = (S,\Delta,\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}) \gets \Gen(n,m)$, and compute $\ket{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
    \item For each $w \in \cW$, derive $x_w,z_w$ from $\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}$ and the circuit topology using the CNOT update rule $(x_1,z_1),(x_2,z_2) \to (x_1,z_1 \oplus z_2),(x_1 \oplus x_2,z_2)$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^n)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^n$. 
    \item For each $i \in [t]$, prepare an oracle $\sF_i^H$ that implements the classical functionality described in \proref{fig:F-oracle}.
    \item Prepare an oracle $\sG^H$ that implements the classical functionality described in \proref{fig:G-oracle}.
    \item Output \[\ket{\widetilde{\psi}},\ket{\sk},\sF_1^H,\dots,\sF_t^H,\sG^H.\]
\end{itemize}

}





   

\protocol{$\sF_i^H$ Functionality}{$\sF_i$}{fig:F-oracle}{
    \begin{itemize}
        \item \textbf{Input:} $\left(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s_{i,0}^M,s_{i,1}^M\right)$
        \item \textbf{Verify $\sigma_x$:} Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item \textbf{Decode $\{\overline{s}_\iota\}_{\iota \in [i]}$:} For each $\iota \in [i]$, $\overline{s}_\iota = \{s_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ is a set of vectors that are supposed to be standard or Hadamard basis measurements of authenticated wires. For $w \in \cW^S_\iota$, define 
        
        \[a_w = \begin{cases} 0 \text{ if } s_w \in S+x_w\\ 1 \text{ if } s_w \in S+\Delta+x_w \\ \bot \text{ else}
        \end{cases},\]

         and for $w \in \cW^H_\iota$, define 

         \[a_w = \begin{cases} 0 \text{ if } s_w \in \widehat{S}+z_w\\ 1 \text{ if } s_w \in \widehat{S}+\widehat{\Delta}+z_w \\ \bot \text{ else}
        \end{cases}.\]
        
        If any were $\bot$, abort and output $\bot$. Otherwise, define $\overline{a}_\iota = \{a_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ for each $\iota \in [i]$.
        \item \textbf{Decode $\{\ell_\iota\}_{\iota \in [i-1]}$:} For each $\iota \in [i-1]$, define the bit $r_\iota=b$ if \[\ell_\iota = H(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota,b),\] and otherwise output $\bot$.
        \item \textbf{Compute next control bit:} Compute $c_i = f_i(x,\overline{a}_1,r_1,\dots,\overline{a}_{i-1},r_{i-1},\overline{a}_i)$.
        \item \textbf{Compute next label:} Parse $\cW_i^M = \{w_0,w_1\}$. For $b \in \{0,1\}$, define \[\ell^b_i = H(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,b).\]If $c_i = 0$, define

        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\} \\
            \bot \text{ else}
        \end{cases}\]

        If $c_i = 1$, define
        
        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\} \\ 
            \bot \text{ else}
        \end{cases}\]

        \item \textbf{Output:} $\ell_i$
   
    \end{itemize}
}

    


\protocol{$\sG^H$ Functionality}{$\sG$}{fig:G-oracle}{
\begin{itemize}
        \item \textbf{Input:} $(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{t-1},\ell_{t},\overline{s}_{t+1})$
        \item \textbf{Check $\sigma_x$:} Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item \textbf{Decode $\{\overline{s}_\iota\}_{\iota \in [t+1]}$:} For each $\iota \in [t+1]$, $\overline{s}_\iota = \{s_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ is a set of vectors that are supposed to be standard or Hadamard basis measurements of authenticated wires. For $w \in \cW^S_\iota$, define 
        
        \[a_w = \begin{cases} 0 \text{ if } s_w \in S+x_w\\ 1 \text{ if } s_w \in S+\Delta+x_w \\ \bot \text{ else}
        \end{cases},\]

         and for $w \in \cW^H_\iota$, define 

         \[a_w = \begin{cases} 0 \text{ if } s_w \in \widehat{S}+z_w\\ 1 \text{ if } s_w \in \widehat{S}+\widehat{\Delta}+z_w \\ \bot \text{ else}
        \end{cases}.\]
        
        If any were $\bot$, abort and output $\bot$. Otherwise, define $\overline{a}_\iota = \{a_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ for each $\iota \in [t+1]$.
        \item \textbf{Decode $\{\ell_\iota\}_{\iota \in [t]}$:} For each $\iota \in [t]$, define the bit $r_\iota=b$ if \[\ell_\iota = H(x,\sigma_x,\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota,b),\] and otherwise output $\bot$.
        \item \textbf{Output:} $y = g(x,\overline{a}_1,r_1,\dots,\overline{a}_t,r_t,\overline{a}_{t+1})$.
    \end{itemize}
    }
        
    


==> old-security-proof.tex <==
First, we describe the simulated state and oracles in \proref{fig:QSim}. Looking ahead, the actual simulator will run the adversary using this simulated information, and output the adversary's final state.

We follow this with the description of a distribution where only the $\sG$ oracle is simulated (\proref{fig:QSimG}), and the description of a distribution where all of the oracles $\sF_1,\dots,\sF_t,\sG$ are simulated, but not the state (\proref{fig:QSimFG}). These distributions will be utilized in the proof.

\protocol{$\QSim$}{Simulated state and oracles, which use oracle access to $Q$.}{fig:QSim}{
    \noindent $\QSim^Q(1^\secp)$:
    \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{0^n})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\FSim_i$ described in \proref{fig:FSim}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output $\ket*{\widetilde{\psi}},\ket{\sk},\FSim_1,\dots,\FSim_t,\GSim^{Q}.$
    \end{itemize}
}

\protocol{$\FSim_i$}{The measurement is verified rather than decoded. The output is always the 0 label.}{fig:FSim}{
$\FSim_i\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$:
    \begin{itemize}
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item For each $\iota \in [i-1]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. 
        \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i) = \bot$. 
        \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},0),$ and output $(\widetilde{v}_i,\ell_i)$.
    \end{itemize}
}

\protocol{$\GSim^Q$}{The measurement is verified rather than decoded. The output is always $Q(x)$.}{fig:GSim}{
$\GSim\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t\right):$
    \begin{itemize}
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item For each $\iota \in [t]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{w}_1,\dots,\widetilde{w}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. 
        \item Output $\bot$ if $\Ver_{k,L_{t+1} \dots L_1,\theta_{t+1}}(\widetilde{v}_1,\dots,\widetilde{v}_{t+1}) = \bot$. 
        \item Output $Q(x)$.
    \end{itemize}
}

\protocol{$\QSimG$}{Only simulate the $\sG$ oracle.}{fig:QSimG}{
    \noindent $\QSim^Q(1^\secp,\ket{\psi})$:
    \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i$ described in \proref{fig:F-oracle}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output $\ket*{\widetilde{\psi}},\ket{\sk},\sF_1,\dots,\sF_t,\GSim^{Q}.$
    \end{itemize}
}

\protocol{$\QSimFG$}{Simulate the $\sF_i$ and $\sG$ oracles, but not the state.}{fig:QSimFG}{
    \noindent $\QSim^Q(1^\secp,\ket{\psi})$:
    \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\FSim_i$ described in \proref{fig:FSim}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output $\ket*{\widetilde{\psi}},\ket{\sk},\FSim_1,\dots,\FSim_t,\GSim^{Q}.$
    \end{itemize}
}













Now, we turn to the security proof. We refer the reader to \cref{subsec:overview-GC} and \cref{subsec:overview-obf} for an overview of the main ideas used in the proof. 


\protocol{$\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$}{The first $\tau$ measurement results on input $x^*$ are hard-coded into the oracles. This distribution is also defined to output a set $B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ which will be referenced in the proof. Note that in the case $\tau = 0$, this distribution on $\ket*{\widetilde{\psi}},\ket{\sk},O$ is identical to that output by $\QSimG$, described in \proref{fig:QSimG}.}{fig:ParMeas}{
    $\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}](1^\secp,\ket{\psi})$:
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ described in \proref{fig:F-ParMeas}.
        \item Let $B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ be the set of $(\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t)$ such that \[\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}](x^*,\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t) \notin \{Q(x^*),\bot\},\] where $\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ is described in \proref{fig:G-ParMeas}. 
        
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  \[\ket*{\widetilde{\psi}},\ket{\sk},O = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\GSim^Q\right), B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}].\]
    \end{itemize}
}

\protocol{$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$}{$\sF_i$ with the first $\tau$ measurement results on input $x^*$ hard-coded.}{fig:F-ParMeas}{
$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$:
    \begin{itemize}
        \item If $x \neq x^*$, output $\sF_i\left(x,\sigma_{x},\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$. 
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.

        \item For each $\iota \in [\min\{\tau,i-1\}]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. 
        
        \item If $i \leq \tau$:
        \begin{itemize}
            
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i) = \bot$. 
             \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r^*_i)$, and output $(\ell_i,\widetilde{v}_i)$. 
        \end{itemize}


        \item If $i > \tau$:
        \begin{itemize}
            
            \item For each $\iota \in [\tau+1,i-1]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. Otherwise, let $r_\iota$ be the bit such that $\ell_\iota = h_{\iota,r_\iota}$.
            \item Define $\theta_i^\Ver = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in (V_{\tau+1},\dots,V_i,W_i)$.
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i^\Ver}(\widetilde{v}_1,\dots,\widetilde{v}_\tau) = \bot$. 
            \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in (V_1,\dots,V_\tau)$.
            \item Compute $(v_{\tau+1},\dots,v_i,w_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_i,\widetilde{w}_i)$, and output $\bot$ if the result was $\bot$.
            \item Compute $(v_i,r_i) = f_i^{x,r^*_1,\dots,r^*_\tau,r_{\tau+1},\dots,r_{i-1}}(v^*_1,\dots,v^*_\tau,v_{\tau+1},\dots,v_i,w_i)$.
             \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r_i)$, and output $(\ell_i,\widetilde{v}_i)$. 
        \end{itemize}

       



        
        
    \end{itemize}
}



\protocol{$\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$}{$\sG$ with the first $\tau$ measurements results on input $x^*$ hard-coded.}{fig:G-ParMeas}{
$\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t\right)$:
        \begin{itemize}
        \item If $x \neq x^*$, output $\sG\left(x,\sigma_{x},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t\right)$. 
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item For each $\iota \in [t]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. If $\iota > \tau$, let $r_\iota$ be the bit such that $\ell_\iota = h_{\iota,r_\iota}$.
        \item Define $\theta_{t+1}^\Ver = \theta_{t+1}$ except that $\theta_{t+1,j}^\Ver = \bot$ for $j \in (V_{\tau+1},\dots,V_{t+1})$.
        \item Output $\bot$ if $\Ver_{k,L_{t+1} \dots L_1,\theta_{t+1}^\Ver}(\widetilde{v}_1,\dots,\widetilde{v}_\tau) = \bot$. 
        \item Define $\theta_{t+1}^\Dec = \theta_{t+1}$ except that $\theta_{t+1,j}^\Dec = \bot$ for $j \in (V_1,\dots,V_\tau)$.
        \item Compute $(v_{\tau+1},\dots,v_{t+1}) = \Dec_{k,L_{t+1}\dots L_1,\theta_{t+1}^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_{t+1})$, and output $\bot$ if the result was $\bot$.
        \item Output $y = g^{x,r^*_1,\dots,r^*_\tau,r_{\tau+1},\dots,r_t}(v_1^*,\dots,v_\tau^*,v_{\tau+1},\dots,v_{t+1}).$
        
    \end{itemize}

}


\protocol{$\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$}{This distribution outputs two sets of oracles - one that corresponds to hard-coding the first $\tau-1$ measurements and one the corresponds to hard-coding the first $\tau$ measurements - along with the set of inputs $\delta$ on which they differ.}{fig:ParMeas-delta}{
    $\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}](1^\secp,\ket{\psi}):$
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}]$ described in \proref{fig:F-ParMeas}, and let $B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}]$ be the set of $(\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t)$ such that \[\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}](x^*,\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t) \notin \{Q(x^*),\bot\}.\]
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ described in \proref{fig:F-ParMeas}, and let $B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ be the set of $(\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t)$ such that \[\sG[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}](x^*,\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_{t+1},\ell_1,\dots,\ell_t) \notin \{Q(x^*),\bot\}.\]
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  \begin{align*}\ket*{\widetilde{\psi}},\ket{\sk}, &O_1 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}],\GSim^Q\right),\\
        &O_2 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\GSim^Q\right), \delta,
        \end{align*}
        where $\delta$ is the set of inputs on which $O_1$ and $O_2$ differ, including \[B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau-1]}] \setminus B[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}].\]
    \end{itemize}
}


\protocol{$\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]$}{The first $\tau$ measurement results and remaining $t-\tau$ magic state values on input $x^*$ are hard-coded into the oracles.}{fig:ParMeas-w-partial}{
    $\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](1^\secp,\ket{\psi}):$
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]$ described in \proref{fig:F-ParMeas-w-partial}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  \begin{align*}
        &\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}],\GSim^Q.
        \end{align*}
    \end{itemize}
}


\protocol{$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]$}{$\sF_i$ with the first $\tau$ measurement results and remaining $t-\tau$ magic state values on input $x^*$ hard-coded.}{fig:F-ParMeas-w-partial}{
$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v_i},\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$:
\begin{itemize}
    \item If $x \neq x^*$, output $\sF_i\left(x,\sigma_{x},\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$. 
    \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
    \item For each $\iota \in [i-1]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. 


 
        
        \item If $i \leq \tau$:
        \begin{itemize}
            
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i) = \bot$. 
            \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r^*_i),$ and output $(\widetilde{v}_i,\ell_i)$.
        \end{itemize}


        \item If $i > \tau$:
        \begin{itemize}
            \item Define $\theta_i^\Ver = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in (V_{\tau+1},\dots,V_i)$.
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i^\Ver}(\widetilde{v}_1,\dots,\widetilde{v}_\tau,\widetilde{w}_i) = \bot$. 
            \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in (V_1,\dots,V_\tau,W_i)$.
            \item Compute $(v_{\tau+1},\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$.
            \item For each $\iota \in [\tau+1,\dots,i]$, compute \[(v_\iota,r_\iota) = f_i^{x,r^*_1,\dots,r^*_\tau,r_{\tau+1},\dots,r_{\iota-1}}(v_1^*,\dots,v_\tau^*,v_{\tau+1},\dots,v_\iota,w^*_\iota).\]
            \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r_i),$ and output $(\widetilde{v}_i,\ell_i)$.


        \end{itemize}

        
        
\end{itemize}

}

\protocol{$\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]$}{This distribution outputs two sets of oracles - one that corresponds to just hard-coding the first $\tau$ measurement results on input $x^*$, and one that additionally hard-codes the remaining $t-\tau$ magic state values - along with the set of points on which they differ.}{fig:ParMeas-w-partial-delta}{
    $\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](1^\secp,\ket{\psi}):$
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ described in \proref{fig:F-ParMeas}.
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]$ described in \proref{fig:F-ParMeas-w-partial}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  \begin{align*}\ket*{\widetilde{\psi}},\ket{\sk}, &O_1 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\GSim^Q\right),\\
        &O_2 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}],\GSim^Q\right), \delta,
        \end{align*}
        where $\delta$ is the set of inputs on which $O_1$ and $O_2$ differ.
    \end{itemize}
}

\protocol{$\ParSim[x^*]$}{The oracles are simulated on input $x^*$.}{fig:ParSim}{

$\ParSim[x^*](1^\secp,\ket{\psi})$:
\begin{itemize}
    \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
    \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*]$ defined as \[\sF_i[x^*](x,\cdot) \coloneqq \begin{cases}\FSim_i(x,\cdot) \text{ if } x = x^*  \\\sF_i(x,\cdot) \text{ else}\end{cases},\] where $\FSim_i$ is described in \proref{fig:FSim} and $\sF_i$ is described in \proref{fig:F-oracle}. 
    \item Prepare an oracle $\GSim^Q$ that implements the classical functionality described in \proref{fig:GSim}.
    \item Output  \[\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*],\dots,\sF_t[x^*],\GSim^Q.\]
\end{itemize}

}



\subsection{Additional Lemmas}





In this section, we prove several lemmas of the following flavor: An adversary is given a state and access to either an oracle $O_1$ or $O_2$ sampled from one of two distributions, and we claim that the adversary can only find an input on which the oracles differ with negligible probability. We often combine these lemmas with \cref{lemma:puncture} in order to switch oracle distributions in the main body of the proof given above. Note that if we want to show the claim when the adversary is given either $O_1$ or $O_2$, it suffices to pick a $b \in \{1,2\}$, and show the claim when the adversary is given $O_b$, because the oracles are identical from the adversary's perspective until they find a differing input.




\subsubsection{Hard-coding $\{w^*_\iota\}_{\iota \in [\tau+1,t]}$ after partial measurements}


Here, $O_1$ is an oracle that hard-codes the first $\tau$ measurements on input $x^*$, and $O_2$ additionally hard-codes all standard basis measurement results on qubits $(W_{\tau+1},\dots,W_t)$ to be used on input $x^*$. The relevant figures for this claim are \proref{fig:ParMeas} (partial measurement on $x^*$), \proref{fig:ParMeas-w-partial} (partial measurement on $x^*$ plus hard-coded $\{w^*_\iota\}_{\iota \in [\tau+1,t]}$), and \proref{fig:ParMeas-w-partial-delta} (their difference).



\begin{lemma}\label{lemma:oi-partial-w}
For any $\tau \in [0,\dots,t+1]$, $n$-qubit state $\ket{\psi}$, input $x^*$, $\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}$, $\{w^*_\iota\}_{\iota \in [\tau+1,t]}$, $\poly(\secp)$-query unitary $U$, and $b \in \{1,2\}$,
\[\E\left[\big\| \Pi[\delta]U^{O_b}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|\right] = 2^{2\tau} \cdot 2^{-\Omega(\kappa)},\] where $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_1,O_2,\delta\right) \gets \ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]\left(1^\secp,\ket{\psi}\right)$.
\end{lemma}

\begin{proof}

We show this for $b=1$. Note that all elements of $\delta$ start with $x^*$ and include at least $i > \tau$ layers of measurement results, so restrict attention to these inputs for the rest of the proof. Define the following function.\\

\noindent\underline{$R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](\widetilde{v}_1,\dots,\widetilde{v}_i)$}
\begin{itemize}
    \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in V_1,\dots,V_\tau,W_i$.
    \item Compute $(v_{\tau+1},\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$. 
    \item For $\iota \in [\tau+1,\dots,i]$, compute \[(\cdot,r_\iota) = f^{x,r_1^*,\dots,r_\tau^*,r_{\tau+1},\dots,r_{\iota-1}}(v^*_1,\dots,v^*_\tau,v_{\tau+1},\dots,v_\iota,w^*_\iota),\] and output $r_i$.
\end{itemize}

By definition of the oracles, $O_1$ and $O_2$ are identical on $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$ if 

\[\forall \ \iota \in [i-1], \ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] and $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$. Thus, for any $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}) \in \delta$, it must be that either

\[\exists \ \iota \in [i-1] \text{ s.t. }\ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] or $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) \neq w^*_i$. However, if the adversary has so far only submitted queries that include $\widetilde{w}_i$ (for some $i > \tau$) such that $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$, then it will not have received any labels \[\ell_\iota = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})),\] and thus can only guess such an $\ell_\iota$ with probability $1/2^\kappa$. Thus, it suffices to show that \[\E\left[\big\| \widetilde{\Pi}_{[\tau+1,t],\overline{\{w^*_\iota\}}_{\iota \in [\tau+1,t]}}U^{O_1}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|^2\right] = 2^{2\tau} \cdot 2^{-\Omega(\kappa)}.\] 


By \cref{lemma:project},

    \begin{align*}
    &\E\left[\big\| \widetilde{\Pi}_{[\tau+1,t],\overline{\{w^*_\iota\}}_{\iota \in [\tau+1,t]}}U^{O_1}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|^2\right]\\
    &\leq 2^{2\tau} \cdot \sum_{\{w^*_\iota\}_{\iota \in [\tau]}}\E\left[\big\|\widetilde{\Pi}_{[\tau+1,t],\overline{\{w^*_\iota\}}_{\iota \in [\tau+1,t]}}U^{O_1}\widetilde{\Pi}_{[\tau],\{w^*_\iota\}_{\iota \in [\tau]}}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right].
    \end{align*}

    Then, for any $w^* = \{w^*_\iota\}_{\iota \in [\tau]} \cup \{w^*_{\iota}\}_{\iota \in [\tau+1,t]}$, define \[\left(\ket*{\widetilde{\psi}},\ket{\sk},O_1[w^*]\right) \gets \ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]\left(1^\secp,\ket{\psi}\right).\] 

    So to complete the proof, 

    \begin{align*}
    &\E\left[\big\|\widetilde{\Pi}_{[i+1,t],\overline{\{w^*_\iota\}}_{\iota \in [\tau+1,t]}}U^{O_1}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk} \big\|^2\right]\\
    &\leq \E\left[\big\|\widetilde{\Pi}_{[i+1,t],\overline{\{w^*_\iota\}}_{\iota \in [\tau+1,t]}}U^{O_1[w^*]}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk} \big\|^2\right] + 2^{-\Omega(\kappa)}\\
    &\leq 2^{-\Omega(\kappa)},
    \end{align*}

    where

    \begin{itemize}
        \item The first inequality follows from \cref{lemma:puncture} and \cref{lemma:oi-full-w}.
        \item The second inequality follows from security of the authentication scheme (\cref{thm:auth-sec}), since $O_1[w^*]$ can be implemented just given oracle access to $\Ver_{k,\cdot,\cdot}(\cdot)$ (see \cref{remark:identical-oracles}).
    \end{itemize}


\end{proof}






\subsubsection{Hard-coding $w^*$ after partial measurements}

Here, $O_1$ is an oracle that hard-codes the first $\tau$ measurements on input $x^*$, and $O_2$ additionally hard-codes all standard basis measurement results on qubits $(W_1,\dots,W_t)$ to be used whenever $x \neq x^*$, and after layer $\tau$ on input $x^*$. The relevant figures for this claim are \proref{fig:ParMeas} (partial measurement on $x^*$), \proref{fig:ParMeas-w} (partial measurement on $x^*$ plus hard-coded $w^*$), and \proref{fig:ParMeas-w-delta} (their difference).

Note that in the case $\tau = 0$, neither oracles have an input $x^*$ or partial measurement results hard-coded. In this case, $O_1$ can equivalently be described by $\QSimG$ (\proref{fig:QSimG}).


\begin{lemma}\label{lemma:oi-full-w}
For any $\tau \in [0,\dots,t+1]$, $n$-qubit state $\ket{\psi}$, input $x^*$, $\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}$, $w^* \in \{0,1\}^{2t}$, $\poly(\secp)$-query unitary $U$, and $b \in \{1,2\}$
\[\E\left[\big\| \Pi[\delta]U^{O_b}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|\right] = 2^{-\Omega(\kappa)},\] where $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_1,O_2,\delta\right) \gets \ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]\left(1^\secp,\ket{\psi}\right)$.
\end{lemma}

\begin{proof}
We show this for $b=2$. Note that all elements of $\delta$ either start with $x \neq x^*$ or start with $x$ but include at least $i > \tau$ layers of measurement results, so restrict attention to these inputs for the rest of the proof. Parse $w^* = \{w^*_\iota\}_{\iota \in [t]}$, and define the following function.\\

\noindent\underline{$R[x^*,\{v^*_\iota,r^*_{\iota}\}_{\iota \in [\tau]}][w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_i)$}
\begin{itemize}
    \item If $x = x^*$:
    \begin{itemize}
        \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in V_1,\dots,V_\tau,W_i$.
        \item Compute $(v_{\tau+1},\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$. 
        \item For $\iota \in [\tau+1,\dots,i]$, compute \[(\cdot,r_\iota) = f^{x,r_1^*,\dots,r_\tau^*,r_{\tau+1},\dots,r_{\iota-1}}(v^*_1,\dots,v^*_\tau,v_{\tau+1},\dots,v_\iota,w^*_\iota),\] and output $r_i$.
    \end{itemize}
    \item If $x \neq x^*$: 
    \begin{itemize}
        \item Compute $(v_1,\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$.
        \item For $\iota \in [i]$, compute $(\cdot,r_\iota) = f^{x,r_1,\dots,r_{\iota-1}}(v_1,\dots,v_\iota,w^*_\iota)$, and output $r_i$.
    \end{itemize}
    
    
    
\end{itemize}

By definition of the oracles, $O_1$ and $O_2$ are identical on $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$ if 
\[\forall \ \iota \in [i-1], \ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] and $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$. Thus, for any $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}) \in \delta$, it must be that either

\[\exists \ \iota \in [i-1] \text{ s.t. }\ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] or $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) \neq w^*_i$. However, if the adversary has so far only submitted queries that include $\widetilde{w}_i$ such that $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$, then it will not have received any labels \[\ell_\iota = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})),\] and thus can only guess such an $\ell_\iota$ with probability $1/2^\kappa$. Thus, it suffices to show that \[\E\left[\big\| \widetilde{\Pi}_{[t],\overline{w}^*}U^{O_2}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|\right] = 2^{-\Omega(\kappa)},\] which follows from security of the authentication scheme (\cref{thm:auth-sec}), since $O_2$ can be implemented just given access to $\Ver_{k,\cdot,\cdot}(\cdot)$ (see \cref{remark:identical-oracles}).

\end{proof}


\subsubsection{Hard-coding $w^*$ after simulating $x^*$}

Here, $O_1$ is an oracle that simulates on input $x^*$ but is honest on all other inputs, and $O_2$ additionally hard-codes all standard basis measurement results on qubits $(W_1,\dots,W_t)$\footnote{Recall from our concrete implementation of a $\LM$ circuit that these qubits correspond to the $T$-gate magic states.} to be used whenever $x \neq x^*$. The relevant figures for this claim are \proref{fig:ParSim} (simulation on $x^*$), \proref{fig:ParSim-w} (simulation on $x^*$ plus hard-coded $w^*$), and  \proref{fig:ParSim-delta} (their difference).


\begin{lemma}\label{lemma:oi-full-w-sim}
For any $n$-qubit state $\ket{\psi}$, input $x^*$, $w^* \in \{0,1\}^{2t}$, $\poly(\secp)$-query unitary $U$, and $b \in \{1,2\}$,
\[\E\left[\big\| \Pi[\delta]U^{O_b}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|\right] = 2^{-\Omega(\kappa)},\] where $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_1,O_2,\delta\right) \gets \ParSim\delta[x^*][w^*]\left(1^\secp,\ket{\psi}\right)$.
\end{lemma}

\begin{proof}
We show this for $b=2$. Note that all elements of $\delta$ start with $x \neq x^*$, so restrict attention to such $x$ for the rest of this proof. Parse $w^* = \{w^*_\iota\}_{\iota \in [t]}$ and define the following function.\\

\noindent \underline{$R[w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_i)$}
\begin{itemize}
    \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in W_i$.
    \item Compute $(v_1,\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_1,\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$.
    \item For $\iota \in [i]$, compute $(\cdot,r_\iota) = f^{x,r_1,\dots,r_{\iota-1}}(v_1,\dots,v_\iota,w^*_\iota)$, and output $r_i$.
\end{itemize}

By definition of the oracles, $O_1$ and $O_2$ are identical on $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$ if 
\[\forall \ \iota \in [i-1], \ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, R[w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] and $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$. Thus, for any $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}) \in \delta$, it must be that either

\[\exists \ \iota \in [i-1] \text{ s.t. }\ell_\iota = H\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})\right),\] or $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) \neq w^*_i$. However, if the adversary has so far only submitted queries that include $\widetilde{w}_i$ such that $\Dec_{k,L_i\dots L_1,W_i}(\widetilde{w}_i) = w^*_i$, then it will not have received any labels \[\ell_\iota = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota},\widetilde{w}_{\iota},\ell_1,\dots,\ell_{\iota-1}, 1-R[w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_{\iota})),\] and thus can only guess such an $\ell_\iota$ with probability $1/2^\kappa$. Thus, it suffices to show that \[\E\left[\big\| \widetilde{\Pi}_{[t],\overline{w}^*}U^{O_2}\widetilde{\Pi}_{[t],w^*}\ket*{\widetilde{\psi}}\ket{\sk}]\big\|\right] = 2^{-\Omega(\kappa)},\] which follows from security of the authentication scheme (\cref{thm:auth-sec}), since $O_2$ can be implemented just given access to $\Ver_{k,\cdot,\cdot}(\cdot)$ (see \cref{remark:identical-oracles}).

\end{proof}




\subsubsection{Identical distributions}


\begin{remark}\label{remark:identical-oracles}
For any $\ket{\psi}$, $x^*, \{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}$, and $w^* \in \{0,1\}^{2t}$, the distributions 
\[\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\GSim^Q \gets \ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](1^\secp,\ket{\psi}),\]

\[\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*][w^*],\dots,\sF_t[x^*][w^*],\GSim^Q \gets \ParSim[x^*][w^*](1^\secp,\ket{\psi}),\]

and    

\[\ket*{\widetilde{\psi}},\ket{\sk},\FSim_1,\dots,\FSim_t,\GSim^Q \gets \QSim(1^\secp,\ket{\psi})\]

are identical, and can all be implemented by an algorithm with oracle access to $\Ver_{k,\cdot,\cdot}(\cdot)$ (as opposed to $k$ or $\Dec_{k,\cdot,\cdot}(\cdot)$). Indeed, the only difference in how these oracles are defined is in how the bit $b$ is determined before querying \[H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1},b).\] In the first case $b = R[x^*, \{v^*_\iota,r^*_\iota\}_{\iota \in \tau}][w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_i)$, in the second $b = R[w^*](x,\widetilde{v}_1,\dots,\widetilde{v}_i)$, and in the third $b = 0$. In each case, the bit $b$ is already determined by the preamble $(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$, and $H$ is never queried on \[H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1},1-b).\] Thus, there is only one defined output label per preamble, so the distribution doesn't change if $b$ is always set to 0.

\end{remark}

\begin{remark}\label{remark:x-identical-oracles}
For any $\ket{\psi}$, $x^*$, $\{v^*_\iota,r^*_\iota\}_{\iota \in \tau}$, and $\{w^*_{\iota}\}_{\iota \in [\tau+1,t]}$, the distributions 
\begin{align*}\ket*{\widetilde{\psi}},\ket{\sk},&\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in \tau},\{w^*_{\iota}\}_{\iota \in [\tau+1,t]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in \tau},\{w^*_{\iota}\}_{\iota \in [\tau+1,t]}],\GSim^Q\\ &\gets \ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in \tau},\{w^*_{\iota}\}_{\iota \in [\tau+1,t]}](1^\secp,\ket{\psi})\end{align*} 
and 
\[\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*],\dots,\sF_t[x^*],\GSim^Q \gets \ParSim[x^*](1^\secp,\ket{\psi})\] 
are identical. Indeed, the only difference in how these oracles are defined is in how the bit $b$ is determined before querying \[H(x^*,\sigma_{x^*},\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1},b).\] In the first case, $b = R[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in \tau},\{w^*_{\iota}\}_{\iota \in [\tau+1,t]}](\widetilde{v}_1,\dots,\widetilde{v}_i)$ and in the second $b=0$. Since $b$ is already determined by the preamble in the first case, the distribution doesn't change if it is always set to 0.
\end{remark}






\subsection{Hard-Coded Oracles}





\protocol{$\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]$}{The first $\tau$ measurement results on input $x^*$ and all magic state values are hard-coded into the oracles.}{fig:ParMeas-w}{
    $\ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](1^\secp,\ket{\psi}):$
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]$ described in \proref{fig:F-ParMeas-w}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  $\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\GSim^Q.$
    \end{itemize}
}

\protocol{$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]$}{$\sF_i$ with the first $\tau$ measurement results on input $x^*$ and all magic state values hard-coded.}{fig:F-ParMeas-w}{
$\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$:
    \begin{itemize}
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item For each $\iota \in [i-1]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$. 
        \item Parse $w^* = \{w^*_\iota\}_{\iota \in [t]}$.
        \item If $x \neq x^*$:
        \begin{itemize}
            \item Define $\theta_i^\Ver = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in (V_1,\dots,V_i)$.
            \item Output $\bot$ if $\Ver_{k,L_i\dots L_1,\theta_i^\Ver}(\widetilde{w}_i) = \bot$.
            \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in W_i$.
            \item Compute $(v_1,\dots,v_i) = \Dec_{k,L_i \dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i)$ and output $\bot$ if the result was $\bot$.
            \item For each $\iota \in [i]$, compute $(v_\iota,r_\iota) = f_\iota^{x,r_1,\dots,r_{\iota-1}}(v_1,\dots,v_\iota,w^*_\iota)$.
            \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r_i),$ and output $(\widetilde{v}_i,\ell_i)$.
        \end{itemize}

        \item If $x = x^*$:

        \begin{itemize}
 
        
        \item If $i \leq \tau$:
        \begin{itemize}
            
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i}(\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i) = \bot$. 
            \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r^*_i),$ and output $(\widetilde{v}_i,\ell_i)$.
        \end{itemize}


        \item If $i > \tau$:
        \begin{itemize}
            \item Define $\theta_i^\Ver = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in (V_{\tau+1},\dots,V_i)$.
            \item Output $\bot$ if $\Ver_{k,L_i \dots L_1,\theta_i^\Ver}(\widetilde{v}_1,\dots,\widetilde{v}_\tau,\widetilde{w}_i) = \bot$. 
            \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in (V_1,\dots,V_\tau,W_i)$.
            \item Compute $(v_{\tau+1},\dots,v_i) = \Dec_{k,L_i\dots L_1,\theta_i^\Dec}(\widetilde{v}_{\tau+1},\dots,\widetilde{v}_i)$, and output $\bot$ if the result was $\bot$.
            \item For each $\iota \in [\tau+1,\dots,i]$, compute \[(v_\iota,r_\iota) = f_i^{x,r^*_1,\dots,r^*_\tau,r_{\tau+1},\dots,r_{\iota-1}}(v^*_1,\dots,v^*_\tau,v_{\tau+1},\dots,v_\iota,w^*_\iota).\]
            \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r_i),$ and output $(\widetilde{v}_i,\ell_i)$.
        \end{itemize}


        \end{itemize}



        
        
    \end{itemize}
}


\protocol{$\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]$}{This distribution outputs two sets of oracles - one that corresponds to just hard-coding the first $\tau$ measurement results on input $x^*$, and one that additionally hard-codes all magic state values - along with the set of points on which they differ.}{fig:ParMeas-w-delta}{
    $\ParMeas\delta[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*](1^\secp,\ket{\psi}):$
     \begin{itemize}
        \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
        \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
        \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]$ described in \proref{fig:F-ParMeas}.
        \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*]$ described in \proref{fig:F-ParMeas-w}.
        \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
        \item Output  \begin{align*}\ket*{\widetilde{\psi}},\ket{\sk}, &O_1 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}],\GSim^Q\right),\\
        &O_2 = \left(\sF_1[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\dots,\sF_t[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}][w^*],\GSim^Q\right), \delta,
        \end{align*}
        where $\delta$ is the set of inputs on which $O_1$ and $O_2$ differ.
    \end{itemize}
}







\protocol{$\ParSim[x^*][w^*]$}{The oracles are simulated on input $x^*$, and all magic state values are hard-coded.}{fig:ParSim-w}{
    $\ParSim[x^*][w^*](1^\secp,\ket{\psi}):$
\begin{itemize}
    \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
    \item For each $i \in [\tau]$, prepare an oracle $\sF_i[x^*][w^*]$ described in \proref{fig:F-ParSim-w}.
    \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
    \item Output  \[\ket*{\widetilde{\psi}},\ket{\sk},\sF_1[x^*][w^*],\dots,\sF_t[x^*][w^*],\GSim^Q.\]
\end{itemize}

}



\protocol{$\sF_i[x^*][w^*]$}{$\sF_i$ with $x^*$ simulated and all magic state values hard-coded.}{fig:F-ParSim-w}{
$\sF_i[x^*][w^*]\left(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1}\right)$:
    \begin{itemize}
        \item If $x = x^*$, output $\FSim_i(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\widetilde{w}_i,\ell_1,\dots,\ell_{i-1})$, where $\FSim_i$ is described in \proref{fig:FSim}.
        \item Output $\bot$ if $\TokVer(\vk,x,\sigma_x) = \bot$.
        \item For each $\iota \in [i-1]$, let \[h_{\iota,0} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},0), h_{\iota,1} = H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_\iota,\ell_1,\dots,\ell_{\iota-1},1),\] and output $\bot$ if $h_{\iota,0} = h_{\iota,1}$ or $\ell_\iota \notin \{h_{\iota,0},h_{\iota,1}\}$.


        \item Define $\theta_i^\Ver = \theta_i$ except that $\theta_{i,j}^\Ver = \bot$ for $j \in (V_1,\dots,V_i)$.
        \item Output $\bot$ if $\Ver_{k,L_i\dots L_1,\theta_i^\Ver}(\widetilde{w}_i) = \bot$.
        \item Define $\theta_i^\Dec = \theta_i$ except that $\theta_{i,j}^\Dec = \bot$ for $j \in W_i$.
        \item Compute $(v_1,\dots,v_i) = \Dec_{k,L_i \dots L_1,\theta_i^\Dec}(\widetilde{v}_1,\dots,\widetilde{v}_i)$ and output $\bot$ if the result was $\bot$.
        \item Parse $w^* = \{w^*_\iota\}_{\iota \in [t]}$. 
        \item For each $\iota \in [i]$, compute $(v_\iota,r_\iota) = f_\iota^{x,r_1,\dots,r_{\iota-1}}(v_1,\dots,v_\iota,w^*_\iota)$.
        \item Set $\ell_i \coloneqq H(x,\sigma_x,\widetilde{v}_1,\dots,\widetilde{v}_i,\ell_1,\dots,\ell_{i-1},r_i),$ and output $(\widetilde{v}_i,\ell_i)$.
   
    \end{itemize}

    
    }



\protocol{$\ParSim\delta[x^*][w^*]$}{This distribution outputs two sets of oracles - one that corresponds to just simulating on input $x^*$, and one that additionally hard-codes all magic state values - along with the set of points on which they differ.}{fig:ParSim-delta}{
$\ParSim\delta[x^*][w^*](1^\secp,\ket{\psi})$:
\begin{itemize}
    \item Sample $k \gets \Gen(1^\kappa,1^n)$, and compute $\ket*{\widetilde{\psi}} = \Enc_k(\ket{\psi})$.
    \item Sample a signature token $(\vk,\ket{\sk}) \gets \TokGen(1^\kappa)$.
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^\kappa$. 
    \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*]$ defined as \[\sF_i[x^*](x,\cdot) \coloneqq \begin{cases}\FSim_i(x,\cdot) \text{ if } x = x^* \\\sF_i(x,\cdot) \text{ else}\end{cases},\] where $\FSim_i$ is described in \proref{fig:FSim} and $\sF_i$ is described in \proref{fig:F-oracle}.  
    \item For each $i \in [t]$, prepare an oracle $\sF_i[x^*][w^*]$ described in \proref{fig:F-ParSim-w}.
    \item Prepare an oracle $\GSim^Q$ described in \proref{fig:GSim}.
    \item Output  
    \begin{align*}
    \ket*{\widetilde{\psi}},\ket{\sk},&O_1 = \left(\sF_1[x^*],\dots,\sF_t[x^*],\GSim^Q\right) \\&O_2 = \left(\sF_1[x^*][w^*],\dots,\sF_t[x^*][w^*],\GSim^Q\right),\delta,\end{align*}
    where $\delta$ is the set of inputs on which $O_1$ and $O_2$ have different outputs.
\end{itemize}


}
















































    










We will first move to a world in which we are simulating all oracle responses on input $x^*$, and then appeal to \cref{lemma:random-measurements} below, which contains the meat of the proof.

Consider any $\{w^*_\iota\}_{\iota \in [\tau+1,t]}$ and the following three distributions (described in \proref{fig:ParMeas}, \proref{fig:ParMeas-w-partial}, and \proref{fig:ParSim}):

\begin{itemize}
    \item $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_{\ParMeas}\right) \gets \ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}]\left(1^\secp,\ket*{\psi_{x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}}}\right)$.
    \item $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_{\ParMeas,\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\right) \gets \ParMeas[x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]},\{w^*_\iota\}_{\iota \in [\tau+1,t]}]\left(1^\secp,\ket*{\psi_{x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}}}\right)$.
    \item $\left(\ket*{\widetilde{\psi}},\ket{\sk},O_{\ParSim}\right) \gets \ParSim[x^*]\left(1^\secp,\ket*{\psi_{x^*,\{v_\iota,r_\iota\}_{\iota \in [\tau]}}}\right)$.
\end{itemize}




By \cref{lemma:project},



\begin{align*}
    &\E\left[\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^{O_\ParMeas}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right] \\
    &\leq 2^{2(t-\tau)} \cdot \sum_{\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\E\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^{O_\ParMeas}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2.
\end{align*}

Then to complete the proof, it holds that for any $\{w^*_\iota\}_{\iota \in [\tau+1,t]}$,

\begin{align*}
    &\E\left[\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^{O_\ParMeas}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right]\\
    &\leq \E\left[\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^{O_{\ParMeas,\{w^*_\iota\}_{\iota \in [\tau+1,t]}}}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right] + 2^{2\tau} \cdot 2^{-\Omega(\kappa)}\\
    &=\E\left[\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^{O_{\ParSim}}\widetilde{\Pi}_{[\tau+1,t],\{w^*_\iota\}_{\iota \in [\tau+1,t]}}\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right]+ 2^{2\tau} \cdot 2^{-\Omega(\kappa)}\\
    &\leq 2^{2t} \cdot 2^{-\Omega(\kappa)},
\end{align*}
where

\begin{itemize}
    \item The first inequality follows from \cref{lemma:puncture} and \cref{lemma:oi-partial-w}.
    \item The following equality follows by definition (see \cref{remark:x-identical-oracles}).
    \item The second inequality follows from \cref{lemma:random-measurements} below.
\end{itemize}


\end{proof}






An overview of the main techniques used in proving the following lemma is given in \cref{subsec:overview-obf}. 

\begin{lemma}\label{lemma:random-measurements}
    For any input $x^*$, $\tau \in [t+1]$, measurement results $\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}$, $(v_\tau,r_\tau) \neq (v^*_\tau,r^*_\tau)$, and $\poly(\secp)$-query unitary, it holds that 
 
    \[\E\left[\big\| \left(\Pi^{x^*}_{\vk} \otimes \widetilde{\Pi}^{x^*,r^*_1,\dots,r^*_{\tau-1}}_{v_{\tau},r_\tau}\right)U^O\ket*{\widetilde{\psi}}\ket{\sk}\big\|^2\right] \leq 2^{2t} \cdot 2^{-\Omega(\kappa)},\] where $\left(\ket*{\widetilde{\psi}},\ket{\sk},O\right)$ are sampled by (\proref{fig:ParSim}) \[\left(\ket*{\widetilde{\psi}},\ket{\sk},\left(\sF_1[x^*],\dots,\sF_t[x^*],\GSim^{Q}\right)\right) \gets \ParSim[x^*]\left(1^\secp,\ket*{\psi_{x^*,\{v^*_\iota,r^*_\iota\}_{\iota \in [\tau]}}}\right).\]
\end{lemma}

\begin{proof}

==> security-GC.tex <==
\section{Security: Garbled Circuit}

First, we'll show that the obfuscation construction is secure if we only allow for evaluation on one input. In other words, that the construction is a secure garbled circuit. In this case, the state $\ket{\psi}$ does not have an input register, and running the universal circuit on $\ket{\psi}$ will produce a deterministic output $y$. Let
\[\QGarble(1^\secp,\ket{\psi}) \to \ket{\widetilde{\psi}},F_1,\dots,F_t,G\]
be the same as $\QObf$ described above except that there is no signature token $\ket{\sk}$, and the oracles will not take $(x,\sigma_x)$ as part of their input and will not run the \textbf{Check token} step.

\paragraph{Simulator.} We define the garbled circuit simulator. \\

\noindent\underline{$\QSim(1^\secp,y)$}

\begin{itemize}
    \item Sample $k = (S,\Delta,\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}) \gets \Gen(n,m)$, and compute $\ket{\widetilde{\psi}^\Sim} = \Enc_k(\ket{0}^{\otimes m})$.
    \item For each $w \in \cW$, derive $x_w,z_w$ from $\{x_w,z_w\}_{w \in \cW^{\mathsf{in}}}$ and the circuit topology using the CNOT update rule $(x_1,z_1),(x_2,z_2) \to (x_1,z_1 \oplus z_2),(x_1 \oplus x_2,z_2)$. 
    \item Sample a random oracle $H : \{0,1\}^* \to \{0,1\}^n$. For any $i \in [t]$ and string $(\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i)$, define a single label:\[\ell_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i} \coloneqq H(\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i).\]
    \item For each $i \in [t]$ prepare an oracle $F_i^\Sim$ that implements the classical functionality described in \proref{fig:F-sim}.

    \protocol{$F_i^\Sim$ Functionality}{$F_i^\Sim$}{fig:F-sim}{
    \begin{itemize}
        \item \textbf{Input:} $\left(\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s^M_{i,0},s^M_{i,1}\right)$
        \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [i]}$:} For each $\iota \in [i]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_\iota \union \cW^H_\iota}$. For each $w \in \cW^S_\iota$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
        \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [i-1]}$:} For each $\iota \in [i-1]$, output $\bot$ if $\ell_\iota \neq \ell_{\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$. Otherwise, continue.
        \item \textbf{Compute next label:} Parse $\cW_i^M = \{w_0,w_1\}$. If $(s^M_{i,0},s^M_{i,1}) \notin \{(S_\Delta + x_{w_0}, S_\Delta + x_{w_1})\}$, output $\bot$. Otherwise, continue. %
        \item \textbf{Output:} $\ell_i := \ell_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i} := H(\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i)$. 
    \end{itemize}
    }

    \item Prepare an oracle $G^\Sim$ that implements the classical functionality described in \proref{fig:G-sim}.

    \protocol{$G^\Sim_y$ Functionality}{$G^\Sim_y$}{fig:G-sim}{
    \begin{itemize}
        \item \textbf{Input:} $(\overline{s}_1,\ell_1,\dots,\overline{s}_{t-1},\ell_t,\overline{s}_{t+1})$.
        \item \textbf{Verify $\{\overline{s}_\iota\}_{\iota \in [t+1]}$}: For each $i \in [t]$, parse $\overline{s}_\iota = \{s_w\}_{s \in \cW^S_i \union \cW^H_i}$. For each $w \in \cW^S_i$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for each $w \in \cW^H_\iota$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
        \item \textbf{Verify $\{\ell_\iota\}_{\iota \in [t]}$}: For each $i \in [t]$, output $\bot$ if $\ell_i \neq \ell_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i}$. Otherwise, continue.
        \item \textbf{Output:} $y$.
    \end{itemize}
    }
    \item Output \[\ket{\widetilde{\psi}^\Sim},F_1^\Sim,\dots,F_t^\Sim,G^\Sim_y.\] %
\end{itemize}

The reason for defining the simulated oracles this way is that they don't actually have to decode any intermediate measurement results. Instead, they just check that the measured string is in the correct support ($S_\Delta + x_w$ for standard basis measurements or $\widehat{S}_{\widehat{\Delta}} + z_w$ for Hadamard basis measurements). Moreover, $M$ measurements are not performed, since $F_i^\Sim$ always outputs a single label instead of one of two labels. Finally, $G^\Sim$ will perform the checks and then just directly output $y$ if they pass, rather than decoding all intermediate and $M$ measurements.

The main point is that we can implement these simulated oracles just given access to the public-verification oracles $V_k$ for the authentication scheme (see \cref{sec:authentication}). We will use this fact throughout the security proof.



\begin{theorem}\label{thm:garbled-circuit}
    Fix $C_1,f_1,C_2,\dots,f_t,_{t+1},g$. For any $\ket{\psi}$ with a deterministic output $y$, and any oracle-aided distinguisher $D$ with $\poly(\secp)$ oracle queries,
    \begin{align*}
    \bigg| &\Pr\left[D^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}} = 1 : \left(\ket{\widetilde{\psi}},F_1,\dots,F_t,G\right) \gets \QGarble(1^\secp,\ket{\psi})\right] \\
    &-\Pr\left[D^{F_1^\Sim,\dots,F_t^\Sim,G^\Sim}\ket{\widetilde{\psi}^\Sim} = 1 : \left(\ket{\widetilde{\psi}^\Sim},F_1^\Sim,\dots,F_t^\Sim,G^\Sim\right) \gets \QSim(1^\secp,y)\right]\bigg| = \negl(\secp).\end{align*}
\end{theorem}

\begin{proof}

During the hybrids, we will split $\ket{\widetilde{\psi}}$ up into orthogonal components corresponding to measuring each of the $T$-gate magic state wires $\{\cW_i^M = (w_{i,0},w_{i,1})\}_{i \in [t]}$ in the standard basis. For each $d \in \{0,1\}^{2t}$, define the set \[\widetilde{d} \coloneqq \bigotimes_{i \in [t], b \in \{0,1\}}S+d_{i,b} \cdot \Delta + x_{w_{i,b}},\] and consider the following sequence of hybrids.







\begin{itemize}
    \item The real experiment.
    \[ \cH_0 = \E\left[\big\|D^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2 \right]\]
    \item Simulate $G$.
    \[\cH_1= \E\left[\big\|D^{F_1,\dots,F_t,G^\Sim}\ket{\widetilde{\psi}}\big\|^2\right]\]
    \item Split $\ket{\widetilde{\psi}}$ into orthogonal components.
    \[\cH_2=\E\left[\sum_{d \in \{0,1\}^{2t}}\big\|D^{F_1,\dots,F_t,G^\Sim}\Pi\left[\widetilde{d}\right]\ket{\widetilde{\psi}}\big\|^2\right]\]
    \item Simulate $F_1,\dots,F_t$.
    \[\cH_3=\E\left[\sum_{d \in \{0,1\}^{2t}}\big\|D^{F_1^\Sim,\dots,F_t^\Sim,G^\Sim}\Pi\left[\widetilde{d}\right]\ket{\widetilde{\psi}}\big\|^2\right]\]
    \item Put $\ket{\widetilde{\psi}}$ back together.
    \[\cH_4=\E\left[\big\|D^{F_1^\Sim,\dots,F_t^\Sim,G^\Sim}\ket{\widetilde{\psi}}\big\|^2\right]\]
    \item Simulate $\ket{\widetilde{\psi}}$. This is the simulated experiment.
    \[\cH_5=\E\left[\big\|D^{F_1^\Sim,\dots,F_t^\Sim,G^\Sim}\ket{\widetilde{\psi}^\Sim}\big\|^2 \right]\]
    
\end{itemize}

The proof follows by combining the following claims, and setting parameters appropriately. 


\begin{claim}
    $|\cH_0-\cH_1| \leq 2^{2mt} \cdot \negl(n)$. %
\end{claim}

\begin{proof}
    This follows directly from \cref{lemma:G-sim}.
\end{proof}

\begin{claim}
    $|\cH_1-\cH_2| \leq 2^{2t} \cdot \negl(n)$.
\end{claim}

\begin{proof}
    This follows from \cref{lemma:map-distinguish} and \cref{lemma:d-mapping}. 
\end{proof}

\begin{claim}
    $|\cH_2-\cH_3| \leq \negl(n)$.
\end{claim}

\begin{proof}
    This follows from \cref{lemma:puncture} and \cref{lemma:d-mapping}.
\end{proof}

\begin{claim}
    $|\cH_3-\cH_4| \leq 2^{2t} \cdot \negl(n)$.
\end{claim}

\begin{proof}
    This follows from \cref{lemma:map-distinguish} and \cref{lemma:d-mapping}. 
\end{proof}

\begin{claim}
    $|\cH_4-\cH_5| \leq \negl(n)$.
\end{claim}

\begin{proof}
    This follows from security of the authentication scheme (\cref{thm:basic-authentication}), since authentication implies hiding. %
\end{proof}


\end{proof}



\begin{lemma}\label{lemma:d-mapping}
Given $\left(\ket{\widetilde{\psi}},F_1,\dots,F_t,G\right) \gets \QGarble(1^\secp,\ket{\psi})$, and $d \in \{0,1\}^{2t}$, let $\widetilde{d}$ be as defined in the proof of \cref{thm:garbled-circuit}. Then for any oracle-aided $U$ with $\poly(\secp)$ queries,
\[\E\left[\big\| \left(\sum_{d' \neq d}\Pi\left[\widetilde{d}'\right]\right)U^{F_1,\dots,F_t,G^\Sim}\Pi\left[\widetilde{d}\right]\ket{\widetilde{\psi}}\big\|^2\right] = \negl(n).\] %
\end{lemma}

\begin{proof}
    This follows by observing that the oracles $F_1,\dots,F_t,G^\Sim$ when restricted to inputs in $\Pi[\widetilde{d}]$ can be simulated given just public-verification oracles $V_k$ for the authentication scheme, and then applying security of the authentication scheme (\cref{thm:basic-authentication}). % 
\end{proof}




\begin{lemma}\label{lemma:G-sim}
Given $\left(\ket{\widetilde{\psi}},F_1,\dots,F_t,G\right) \gets \QGarble(1^\secp,\ket{\psi})$, define the set \[\mathsf{bad} \coloneqq \{(\overline{s}_1,\ell_1,\dots,\overline{s}_{t-1},\ell_t,\overline{s}_{t+1}) : G(\overline{s}_1,\ell_1,\dots,\overline{s}_{t-1},\ell_t,\overline{s}_{t+1}) \notin \{y,\bot\}.\] 
Then for any oracle-aided $U$ with $\poly(\secp)$ queries, \[\E\left[\big\|\Pi[\mathsf{bad}]U^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2\right] =  2^{2mt} \cdot \negl(n).\] 
\end{lemma}

%

\begin{proof}

We will show this by induction on $t$. Call the claim in the lemma statement Claim 1. That is,\[\E\left[\big\|\Pi[\mathsf{bad}]U^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2\right] =  2^{2mt} \cdot \negl(n).\tag{Claim 1}
\]

To help with the inductive step, we will also show the following Claim 2. For any BB84 state projector (see \cref{sec:authentication}) $\Pi_{A,\theta}$ such that $\Pi_{A,\theta}\ket{\psi} = 0$, it holds that \[\E\left[\big\|\Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2\right] = 2^{2mt} \cdot \negl(n), \tag{Claim 2}\] where the set $\widetilde{P}_{k,A,\theta}$ is defined based on $\Pi_{A,\theta}$ and the authentication key $k$ as described in \cref{sec:authentication}. \\



\noindent\underline{Base case}\\

When $t=0$, we only have $\left(\ket{\widetilde{\psi}},G\right)$. To show Claim 1, it suffices to show that 

\[\E\left[\big\|\Pi[\mathsf{bad}]U^{G^\Sim}\ket{\widetilde{\psi}}\big\|^2\right] = \negl(n),\]
because $G$ and $G^\Sim$ are identical outside of $\mathsf{bad}$. This then follows directly from \cref{thm:basic-authentication}. To show Claim 2, it now suffices to show that 

\[\E\left[\big\|\Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{G^\Sim}\ket{\widetilde{\psi}}\big\|^2\right] = \negl(n),\] which again follows directly from \cref{thm:basic-authentication}.\\







\noindent\underline{Inductive step: Claim 1}\\

Let's first show Claim 1. We will split $\ket{\widetilde{\psi}}$ up into orthogonal components corresponding to the logical measurement results on wires $\cW_1^S,\cW_1^H,\cW_1^M$. Given $\overline{a}_1 = \{a_w\}_{w \in \cW_1^S \union \cW_1^H},r_1 \in \{0,1\}$, let $\theta$ be the binary string of basis choices indexed by $w \in \cW_1^S \cup \cW_1^H \cup \cW_1^M$ with $\{\theta_w = 0\}_{w \in \cW_1^S \cup \cW_1^M}$ and $\{\theta_w = 1\}_{w \in \cW_1^H}$, and let $A[\overline{a}_1,r_1]$ be the set of two strings $\{\overline{a}_1\} \otimes M_{f_1(\overline{a}_1),r_1}$, where 







 





\[M_{0,0} = \{00,10\}, M_{0,1} = \{01,11\}, M_{1,0} = \{00,11\}, M_{1,1} = \{01,10\}.\]

Additionally given the authentication key $k$, define the set $\widetilde{P}_{k,A[\overline{a}_1,r_1],\theta}$ as in \cref{sec:authentication}. We will actually drop the $\theta$ for notational clarity, and refer to this set as $\widetilde{P}_{k,A[\overline{a}_1,r_1]}$ To be concrete,

\[\widetilde{P}_{k,A[\overline{a}_1,r_1]} \coloneqq \bigotimes_{w \in \cW_1^S} (S + a_w \cdot \Delta + x_w) \bigotimes_{w \in \cW_1^H} (\widehat{S} + a_w \cdot \widehat{\Delta} + z_w) \otimes \bigcup_{a_M \in M_{f_1(\overline{a}_1),r_1}}(S + a_{M,0} \cdot \Delta + x_{w_{M,0}}) \otimes (S + a_{M,1} \cdot \Delta + x_{w_{M,1}}).\] 






Next, given a measurement result $(\overline{a}_1,r_1)$, we define a simulated $F_1^\Sim[r_1]$ in \proref{fig:F1-sim} and partially simulated oracles $F_i^{\ParSim}[\overline{a}_1,r_1]$ in \proref{fig:parsim}, where the differences with $F_i$ are highlighted in red. These oracles will not decode the first set of measurement results, and instead will have $(\overline{a}_1,r_1)$ hard-coded.

\protocol{$F_1^\Sim[r_1]$ Functionality}{$F_1^\Sim[r_1]$}{fig:F1-sim}{
\begin{itemize}
    \item \textbf{Input:} $(\overline{s}_1,s^M_{1,0},s^M_{1,1})$
    \item \textbf{Verify $\overline{s}_1$:} Parse $\overline{s}_1 = \{s_w\}_{w \in \cW_1^S \union \cW_1^H}$. For $w \in \cW_1^S$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for $w \in \cW_1^H$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise, continue.
    \item \textbf{Compute next label:} Parse $\cW_1^M= (w_0,w_1)$. If $(s^M_{1,0},s^M_{1,1}) \notin \{(S_\Delta + x_{w_0},S_\Delta + x_{w_1})\}$, output $\bot$. Otherwise, continue with $\ell_1 = \ell_{\overline{s}_1}^{r_1}$
    \item \textbf{Output:} $\ell_1$.
\end{itemize}


}

\protocol{$F_i^\ParSim[\overline{a}_1,r_1]$ Functionality}{$F_i^\ParSim[\overline{a}_1,r_1]$}{fig:parsimold}{

\begin{itemize}
        \item \textbf{Input:} $(\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i,s^M_{i,0},s^M_{i,1})$
        \item \textcolor{red}{\textbf{Verify} $\overline{s}_1$: Parse $\overline{s}_1 = \{s_w\}_{w \in \cW_1^S \union \cW_1^H}$. For $w \in \cW_1^S$, output $\bot$ if $s_w \notin S_\Delta + x_w$ and for $w \in \cW_1^H$, output $\bot$ if $s_w \notin \widehat{S}_{\widehat{\Delta}} + z_w$. Otherwise continue, using the hard-coded value $\overline{a}_1$.}
        \item \textbf{Decode $\{\overline{s}_\iota\}_{\iota \in \textcolor{red}{[2,\dots,i]}}$:} For each $\iota \in \textcolor{red}{[2,\dots,i]}$, $\overline{s}_\iota = \{s_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ is a set of vectors that are supposed to be standard or Hadamard basis measurements of authenticated wires. For $w \in \cW^S_\iota$, define 
        
        \[a_w = \begin{cases} 0 \text{ if } s_w \in S+x_w\\ 1 \text{ if } s_w \in S+\Delta+x_w \\ \bot \text{ else}
        \end{cases},\]

         and for $w \in \cW^H_\iota$, define 

         \[a_w = \begin{cases} 0 \text{ if } s_w \in \widehat{S}+z_w\\ 1 \text{ if } s_w \in \widehat{S}+\widehat{\Delta}+z_w \\ \bot \text{ else}
        \end{cases},\]
        
        If any were $\bot$, abort and output $\bot$. Otherwise, define $\overline{a}_\iota = \{a_w\}_{w \in \cW^S_\iota \union \cW^H_\iota}$ for each $\iota \in [i]$.

        \item \textcolor{red}{\textbf{Verify $\ell_1$}: If $\ell_1 \neq \ell^{r_1}_{\overline{s}_1}$, output $\bot$. Otherwise continue, using the hard-coded value $r_1$.}
        
        \item \textbf{Decode $\{\ell_\iota\}_{\iota \in \textcolor{red}{[2,\dots,i-1]}}$:} For each $\iota \in \textcolor{red}{[2,\dots,i-1]}$, define the bit $r_\iota=b$ if $\ell_\iota = \ell^b_{\overline{s}_1,\ell_1,\dots,\overline{s}_{\iota-1},\ell_{\iota-1},\overline{s}_\iota}$, and otherwise abort and output $\bot$.
        \item \textbf{Compute next control bit:} Compute $c_i = f_i(\overline{a}_1,r_1,\dots,\overline{a}_{i-1},r_{i-1},\overline{a}_i)$.
        \item \textbf{Compute next label:} For $b \in \{0,1\}$, define $\ell^b_i =\ell^b_{\overline{s}_1,\ell_1,\dots,\overline{s}_{i-1},\ell_{i-1},\overline{s}_i}$, and parse $\cW_i^M = \{w_0,w_1\}$. If $c_i = 0$, define

        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\} \\
            \bot \text{ else}
        \end{cases},\]

        and if $c_i = 1$, define
        
        \[\ell_i = \begin{cases}
            \ell^0_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+x_{w_1}),(S+\Delta+x_{w_0},S+\Delta+x_{w_1})\}  \\ 
            \ell^1_i \text{ if } (s^M_{i,0},s^M_{i,1}) \in \{(S+x_{w_0},S+\Delta+x_{w_1}),(S+\Delta+x_{w_0},S+x_{w_1})\} \\ 
            \bot \text{ else}
        \end{cases}.\]

        \item \textbf{Output:} $\ell_i$
   
    \end{itemize}


}






Now it holds that

\begin{align*}
    &\E\left[\big\|\Pi[\mathsf{bad}]U^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2\right] \\
    &\leq 2^{2m} \cdot \E\left[\sum_{\overline{a}_1,r_1}\big\|\Pi[\mathsf{bad}]U^{F_1,\dots,F_t,G}\Pi\left[\widetilde{P}_{k,A[\overline{a}_1,r_1]}\right]\ket{\widetilde{\psi}}\big\|^2\right] \\
    &\leq 2^{2m} \cdot \Bigg(\E\left[\sum_{\overline{a}_1,r_1}\big\|\Pi[\mathsf{bad}]U^{F_1^\Sim[r_1],F_2^\ParSim[\overline{a}_1,r_1],\dots,F_t^\ParSim[\overline{a}_1,r_1],G^\ParSim[\overline{a}_1,r_1]}\Pi\left[\widetilde{P}_{k,A[\overline{a}_1,r_1]}\right]\ket{\widetilde{\psi}}\Big\|^2\right] \\
    & ~~~~~~~~~~~~~~~~~~ + 2^{2m(t-1)} \cdot \negl(n)\bigg)\\
    &\leq 2^{2mt} \cdot \negl(n),
\end{align*}

where

\begin{itemize}
    \item The first inequality follows from \cref{lemma:project}.
    \item The second inequality follows from \cref{lemma:puncture} and Claim 2 of the induction hypothesis.
    
    To see this, we will first define a particular set of inputs such that the set of oracles $(F_1,\dots,F_t,G)$ and $(F_1^\Sim[r_1],F_2^\ParSim[\overline{a}_1,r_1],\dots,F_t^\ParSim[\overline{a}_1,r_1],G^\ParSim[\overline{a}_1,r_1])$ are identical outside this set. 
    
    \begin{itemize}
        \item First, let $m_1 \coloneqq |\cW_1^S \union \cW_1^H \union \cW_1^M|$ and note that $F_1$ and $F_1^\Sim[r_1]$ are identical outside of $\widetilde{P}_{k,\{0,1\}^{m_1} \setminus A[\overline{a}_1,r_1]}$.
        \item Next, note that $(F_2,\dots,F_t,G)$ and $(F_2^\ParSim[\overline{a}_1,r_1],\allowbreak\dots,\allowbreak F_t^\ParSim[\overline{a}_1,r_1],\allowbreak G^\ParSim[\overline{a}_1,r_1])$ are identical outside of
        \[\widetilde{P}_{k,\{0,1\}^{m_1-2}\setminus\{\overline{a}_1\}} \bigcup \left\{(\overline{s}_1,\ell_{\overline{s}_1}^{1-r_1}) : \overline{s}_1 \in \widetilde{P}_{k,\{\overline{a}_1\}}\right\}\]
    \end{itemize}
    
    
    
    
    

    Now, note that if $F_1^\Sim$ is never queried on a string in $\widetilde{P}_{k,\{0,1\}^{m_1} \setminus A[\overline{a}_1,r_1]}$, then no $\ell_{\overline{s}_1}^{1-r_1}$ is ever returned to the adversary. Thus, since any $\ell_{\overline{s}_1}^{1-r_1}$ can only be guessed with $\negl(n)$ probability, by \cref{lemma:puncture} it suffices to show that for any $(\overline{a}_1,r_1)$,

    \begin{align*}&\E\left[\big\|\Pi\left[\widetilde{P}_{k,\{0,1\}^{m_1} \setminus A[\overline{a}_1,r_1]}\right]U^{F_1^\Sim[r_1],F_2^\ParSim[\overline{a}_1,r_1],\dots,F_t^\ParSim[\overline{a}_1,r_1],G^\ParSim[\overline{a}_1,r_1]}
    \Pi\left[\widetilde{P}_{k,A[\overline{a}_1,r_1]}\right]\ket{\widetilde{\psi}}\big\|^2\right]\\ &\leq 2^{2m(t-1)} \cdot \negl(n).\end{align*}

    However, since the partially simulated oracles can be seen as a $t-1$ layer garbled circuit , this follows from Claim 2 of the induction hypothesis.
    
    
    
    
    
    
    
    
    
    
    


    \item The third inequality follows from Claim 1 of the induction hypothesis.
    

\end{itemize}


\noindent\underline{Inductive Step: Claim 2}\\

For this claim, we will split $\ket{\widetilde{\psi_k}}$ up into orthogonal components corresponding to measuring each of the $\{\cW_i^M = (w_{i,0},w_{i,1})\}_{i \in [t]}$ wires in the standard basis. For each $d \in \{0,1\}^{2t}$, define $\widetilde{d}$ as in the proof of \cref{thm:garbled-circuit}, and let $\Pi_{A,\theta}$ be an BB84 states projector such that $\Pi_{A,\theta}\ket{\psi} = 0$. Then it holds that





\begin{align*}
    &\E\left[\big\| \Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{F_1,\dots,F_t,G}\ket{\widetilde{\psi}}\big\|^2\right]\\ 
    &\leq \E\left[\big\| \Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{F_1,\dots,F_t,G^\Sim}\ket{\widetilde{\psi}}\big\|^2\right] + 2^{2mt} \cdot \negl(n)\\
    &\leq 2^{4t} \cdot \E\left[\sum_{d \in \{0,1\}^{2t}}\big\| \Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{F_1,\dots,F_t,G^\Sim}\Pi\left[\widetilde{d}\right]\ket{\widetilde{\psi}}\big\|^2\right] + 2^{2mt} \cdot \negl(n) \\
    &\leq 2^{4t} \cdot \left(\E\left[\sum_{d \in \{0,1\}^{2t}}\big\| \Pi\left[\widetilde{P}_{k,A,\theta}\right]U^{F_1^\Sim,\dots,F_t^\Sim,G^\Sim}\Pi\left[\widetilde{d}\right]\ket{\widetilde{\psi}}\big\|^2\right] + \negl(n)\right) + 2^{2mt} \cdot \negl(n)\\
    &\leq 2^{2mt} \cdot \negl(n),
\end{align*}

where

\begin{itemize}
    \item The first inequality follows from Claim 1 shown above.
    \item The second inequality follows from \cref{lemma:project}.
    \item The third inequality follows from \cref{lemma:puncture} and \cref{lemma:d-mapping}. 
    
    
    
    \item The fourth inequality follows from the security of the authentication scheme (\cref{thm:basic-authentication}). %
    
    
\end{itemize}

\end{proof}








